AdaMatch: A Unified Approach to Semi-Supervised Learning and Domain Adaptation

We extend semi-supervised learning to the problem of domain adaptation to learn significantly higher-accuracy models that train on one data distribution and test on a different one. With the goal of generality, we introduce AdaMatch, a method that unifies the tasks of unsupervised domain adaptation (UDA), semi-supervised learning (SSL), and semi-supervised domain adaptation (SSDA). In an extensive experimental study, we compare its behavior with respective state-of-the-art techniques from SSL, SSDA, and UDA on vision classification tasks. We find AdaMatch either matches or significantly exceeds the state-of-the-art in each case using the same hyper-parameters regardless of the dataset or task. For example, AdaMatch nearly doubles the accuracy compared to that of the prior state-of-the-art on the UDA task for DomainNet and even exceeds the accuracy of the prior state-of-the-art obtained with pre-training by 6.4% when AdaMatch is trained completely from scratch. Furthermore, by providing AdaMatch with just one labeled example per class from the target domain (i.e., the SSDA setting), we increase the target accuracy by an additional 6.1%, and with 5 labeled examples, by 13.6%.

==> AdaMatch - ICLR 2022/autogenerated_figures.tex <==
% ['data/NextMatch Results - DA.csv', 'data/NextMatch Results - DA - DigitFive.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrr}
\toprule
& DigitFive     & DomainNet64   & DomainNet224  \\
& 1     & 1     & 1     \\
\\
\midrule
BaselineBN      & nan   & 15.8  & 18.9  \\
MCD             & 57.8  & 14.9  & 14.9  \\
NoisyStudent    & 73.3  & 21.0  & 23.6  \\
FixMatch+       & 92.9  & 21.6  & 21.3  \\
AdaMatch        & 97.8  & 26.0  & 28.7  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


% ['data/NextMatch Results - SSL.csv', 'data/NextMatch Results - SSL - DigitFive.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive     & DigitFive     & DigitFive     & DigitFive     & DomainNet64   & DomainNet64   & DomainNet64   & DomainNet64   & DomainNet224  & DomainNet224  & DomainNet224  & DomainNet224  \\
& 1     & 25    & 5     & 10    & 10    & 5     & 1     & 25    & 10    & 5     & 1     & 25    \\
\\
\midrule
BaselineBN      & nan   & nan   & nan   & nan   & 23.9  & 16.5  & 5.9   & 34.9  & 26.2  & 18.1  & 6.5   & 38.5  \\
MCD             & 27.4  & 93.0  & 50.8  & 78.4  & 16.7  & 10.2  & 3.1   & 27.5  & 14.9  & 8.9   & 2.8   & 26.0  \\
NoisyStudent    & 43.3  & 92.1  & 67.4  & 80.5  & 29.3  & 21.1  & 7.3   & 40.3  & nan   & nan   & nan   & nan   \\
FixMatch+       & 60.8  & 98.2  & 95.0  & 98.3  & 32.3  & 24.1  & 7.7   & 41.3  & 32.8  & 23.8  & 7.6   & 43.0  \\
AdaMatch        & 68.6  & 97.6  & 97.2  & 97.6  & 31.7  & 23.8  & 8.1   & 41.4  & 34.9  & 25.7  & 8.2   & 46.4  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


% data/NextMatch Results - SSDA.csv
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
& \multicolumn{4}{c}{DomainNet64}  & \multicolumn{4}{c}{DomainNet224} \\
& 5     & 25    & 10    & 1     & 25    & 5     & 1     & 10    \\
\\
\midrule
BaselineBN      & 28.6  & 42.1  & 34.0  & 20.8  & 47.6  & 33.8  & 25.3  & 39.3  \\
MCD             & 19.5  & 33.2  & 24.3  & 13.8  & 32.5  & 17.8  & 13.5  & 23.1  \\
NoisyStudent    & 28.6  & 41.4  & 33.6  & 22.8  & nan   & nan   & nan   & nan   \\
FixMatch+       & 37.0  & 47.4  & 41.8  & 28.2  & 51.0  & 41.5  & 31.0  & 46.7  \\
AdaMatch        & 36.5  & 46.4  & 40.6  & 30.4  & 52.8  & 42.3  & 34.8  & 46.7  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


==> AdaMatch - ICLR 2022/latexdefs.tex <==
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\fhat}{\ensuremath{\hat{f}}}
\newcommand{\ermloss}{\ensuremath{L}}
\newcommand{\Eop}{\ensuremath{\mathop{\mathbb{E}}}}
\newcommand{\E}{\Eop}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Dtest}{\ensuremath{S}}
\newcommand{\D}[1]{\ensuremath{D_{\text{#1}}}}
\newcommand{\ind}{\ensuremath{\mathbb{I}}}
\newcommand{\acc}{\ensuremath{\text{acc}}}
\newcommand{\Beta}{\ensuremath{\text{Beta}}}
\newcommand{\Uniform}{\ensuremath{\text{Uniform}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\newcommand{\fixmatchda}{FixMatch+}
\newcommand{\baselinebn}{BaselineBN}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}


\iftoggle{showtodos}{
\newcommand{\becca}[1]{\todo[color=green!40]{Becca: #1}}
\newcommand{\david}[1]{\todo[color=blue!40]{David: #1}}
\newcommand{\nicholas}[1]{\todo[color=red!40]{Nicholas: #1}}
\newcommand{\kihyuk}[1]{\todo[color=purple!40]{Kihyuk: #1}}
\newcommand{\alex}[1]{\todo[color=purple!40]{Alex: #1}}
}{
\newcommand{\becca}[1]{}
\newcommand{\david}[1]{}
\newcommand{\nicholas}[1]{}
\newcommand{\kihyuk}[1]{}
\newcommand{\alex}[1]{}
}


% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }

==> AdaMatch - ICLR 2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> AdaMatch - ICLR 2022/new-06-03.tex <==
%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive AdaMatch (num\_target\_labels=1)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.1	& 96.7	& 99.4	& 97.8	& 98.3	\\
mnistm  	& 99.5	& -	& 96.8	& 99.7	& 97.9	& 98.5	\\
svhn    	& 99.2	& 98.9	& -	& 99.6	& 90.7	& 97.1	\\
syndigit	& 99.3	& 98.9	& 97.0	& -	& 97.1	& 98.1	\\
usps    	& 99.3	& 98.9	& 96.6	& 95.0	& -	& 97.4	\\
\midrule
Avg	& 99.3	& 98.9	& 96.8	& 98.4	& 95.9	& 97.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive AdaMatch (num\_target\_labels=5)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.7	& 99.5	& 97.8	& 98.3	\\
mnistm  	& 99.5	& -	& 96.7	& 99.7	& 97.7	& 98.4	\\
svhn    	& 99.3	& 98.9	& -	& 99.5	& 94.5	& 98.0	\\
syndigit	& 99.3	& 98.9	& 96.8	& -	& 97.0	& 98.0	\\
usps    	& 99.4	& 99.0	& 96.1	& 95.5	& -	& 97.5	\\
\midrule
Avg	& 99.4	& 99.0	& 96.6	& 98.5	& 96.8	& 98.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive AdaMatch (num\_target\_labels=10)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.7	& 99.7	& 97.7	& 98.3	\\
mnistm  	& 99.4	& -	& 96.6	& 99.7	& 97.7	& 98.3	\\
svhn    	& 99.3	& 98.8	& -	& 99.6	& 91.5	& 97.3	\\
syndigit	& 99.3	& 99.0	& 96.9	& -	& 97.4	& 98.2	\\
usps    	& 99.4	& 98.9	& 83.5	& 95.6	& -	& 94.3	\\
\midrule
Avg	& 99.3	& 99.0	& 93.4	& 98.7	& 96.1	& 97.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive AdaMatch (num\_target\_labels=25)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.1	& 99.4	& 97.9	& 98.2	\\
mnistm  	& 99.4	& -	& 96.4	& 98.7	& 97.9	& 98.1	\\
svhn    	& 99.3	& 98.7	& -	& 99.6	& 96.8	& 98.6	\\
syndigit	& 99.3	& 98.8	& 96.4	& -	& 97.6	& 98.0	\\
usps    	& 99.3	& 98.9	& 83.8	& 99.3	& -	& 95.3	\\
\midrule
Avg	& 99.3	& 98.9	& 93.2	& 99.3	& 97.6	& 97.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive BaselineBN (num\_target\_labels=1)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 72.8	& 42.1	& 78.3	& 95.8	& 72.2	\\
mnistm  	& 97.1	& -	& 60.6	& 86.5	& 94.8	& 84.8	\\
svhn    	& 76.5	& 37.0	& -	& 97.3	& 63.6	& 68.6	\\
syndigit	& 85.7	& 31.1	& 77.0	& -	& 80.3	& 68.5	\\
usps    	& 83.5	& 33.0	& 31.7	& 70.3	& -	& 54.6	\\
\midrule
Avg	& 85.7	& 43.5	& 52.8	& 83.1	& 83.6	& 69.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive BaselineBN (num\_target\_labels=5)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 79.7	& 59.4	& 90.0	& 96.4	& 81.4	\\
mnistm  	& 96.5	& -	& 68.4	& 91.4	& 95.7	& 88.0	\\
svhn    	& 90.6	& 49.1	& -	& 97.4	& 82.8	& 80.0	\\
syndigit	& 91.5	& 50.8	& 80.0	& -	& 87.4	& 77.4	\\
usps    	& 91.3	& 45.5	& 48.0	& 84.8	& -	& 67.4	\\
\midrule
Avg	& 92.5	& 56.3	& 64.0	& 90.9	& 90.6	& 78.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive BaselineBN (num\_target\_labels=10)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 85.6	& 68.3	& 92.2	& 96.9	& 85.8	\\
mnistm  	& 98.2	& -	& 75.6	& 93.0	& 95.2	& 90.5	\\
svhn    	& 94.8	& 65.3	& -	& 97.4	& 89.4	& 86.7	\\
syndigit	& 95.9	& 68.1	& 83.5	& -	& 92.2	& 84.9	\\
usps    	& 94.3	& 65.0	& 61.3	& 89.1	& -	& 77.4	\\
\midrule
Avg	& 95.8	& 71.0	& 72.2	& 92.9	& 93.4	& 85.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive BaselineBN (num\_target\_labels=25)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 93.2	& 76.8	& 95.8	& 97.1	& 90.7	\\
mnistm  	& 98.8	& -	& 79.3	& 95.8	& 96.8	& 92.7	\\
svhn    	& 96.8	& 83.2	& -	& 98.2	& 94.9	& 93.3	\\
syndigit	& 97.0	& 84.7	& 86.4	& -	& 95.6	& 90.9	\\
usps    	& 96.8	& 84.8	& 72.2	& 94.5	& -	& 87.1	\\
\midrule
Avg	& 97.4	& 86.5	& 78.7	& 96.1	& 96.1	& 90.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 54.5	& 99.7	& 98.1	& 87.9	\\
mnistm  	& 99.4	& -	& 54.7	& 99.7	& 97.8	& 87.9	\\
svhn    	& 97.9	& 10.9	& -	& 99.6	& 97.3	& 76.4	\\
syndigit	& 99.4	& 98.8	& 97.1	& -	& 97.4	& 98.2	\\
usps    	& 99.3	& 9.8	& 28.8	& 99.7	& -	& 59.4	\\
\midrule
Avg	& 99.0	& 54.7	& 58.8	& 99.7	& 97.7	& 82.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 80.8	& 99.7	& 98.0	& 94.4	\\
mnistm  	& 99.4	& -	& 86.7	& 99.3	& 97.8	& 95.8	\\
svhn    	& 97.9	& 97.4	& -	& 99.6	& 93.2	& 97.0	\\
syndigit	& 99.3	& 98.9	& 96.9	& -	& 97.7	& 98.2	\\
usps    	& 99.3	& 99.0	& 96.8	& 99.7	& -	& 98.7	\\
\midrule
Avg	& 99.0	& 98.6	& 90.3	& 99.6	& 96.7	& 96.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.7	& 99.7	& 97.9	& 98.4	\\
mnistm  	& 99.5	& -	& 97.0	& 99.8	& 97.7	& 98.5	\\
svhn    	& 99.3	& 98.8	& -	& 99.6	& 97.3	& 98.8	\\
syndigit	& 99.3	& 98.9	& 97.2	& -	& 97.3	& 98.2	\\
usps    	& 99.4	& 98.9	& 96.8	& 99.7	& -	& 98.7	\\
\midrule
Avg	& 99.4	& 98.9	& 96.9	& 99.7	& 97.6	& 98.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.5	& 99.8	& 97.8	& 98.3	\\
mnistm  	& 99.5	& -	& 96.5	& 99.8	& 97.5	& 98.3	\\
svhn    	& 99.2	& 98.7	& -	& 99.6	& 97.5	& 98.8	\\
syndigit	& 99.4	& 98.8	& 96.6	& -	& 97.5	& 98.1	\\
usps    	& 99.3	& 98.9	& 96.4	& 99.8	& -	& 98.6	\\
\midrule
Avg	& 99.4	& 98.9	& 96.5	& 99.8	& 97.6	& 98.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive MCD (num\_target\_labels=1)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 70.8	& 12.2	& 21.7	& 96.6	& 50.3	\\
mnistm  	& 98.7	& -	& 7.7	& 87.9	& 94.3	& 72.2	\\
svhn    	& 93.2	& 62.8	& -	& 98.0	& 92.4	& 86.6	\\
syndigit	& 98.2	& 70.6	& 83.7	& -	& 94.9	& 86.8	\\
usps    	& 98.3	& 10.0	& 10.8	& 27.9	& -	& 36.8	\\
\midrule
Avg	& 97.1	& 53.5	& 28.6	& 58.9	& 94.5	& 66.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using MCD.}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive MCD (num\_target\_labels=5)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 69.7	& 14.2	& 81.7	& 96.5	& 65.5	\\
mnistm  	& 98.5	& -	& 7.6	& 88.3	& 95.1	& 72.4	\\
svhn    	& 97.6	& 65.9	& -	& 98.1	& 91.5	& 88.3	\\
syndigit	& 98.5	& 87.9	& 84.7	& -	& 94.9	& 91.5	\\
usps    	& 97.9	& 61.0	& 9.8	& 91.1	& -	& 65.0	\\
\midrule
Avg	& 98.1	& 71.1	& 29.1	& 89.8	& 94.5	& 76.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using MCD.}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive MCD (num\_target\_labels=10)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 76.6	& 7.3	& 95.4	& 96.4	& 68.9	\\
mnistm  	& 98.7	& -	& 13.5	& 95.9	& 95.5	& 75.9	\\
svhn    	& 97.6	& 91.1	& -	& 98.3	& 94.2	& 95.3	\\
syndigit	& 98.6	& 94.4	& 85.9	& -	& 95.3	& 93.5	\\
usps    	& 98.3	& 73.2	& 10.7	& 95.3	& -	& 69.4	\\
\midrule
Avg	& 98.3	& 83.8	& 29.4	& 96.2	& 95.4	& 80.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using MCD.}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive MCD (num\_target\_labels=25)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 97.5	& 64.8	& 96.8	& 95.9	& 88.8	\\
mnistm  	& 99.0	& -	& 23.7	& 97.2	& 95.6	& 78.9	\\
svhn    	& 98.1	& 93.1	& -	& 98.3	& 95.0	& 96.1	\\
syndigit	& 98.0	& 96.0	& 87.1	& -	& 95.3	& 94.1	\\
usps    	& 98.5	& 93.5	& 77.0	& 97.0	& -	& 91.5	\\
\midrule
Avg	& 98.4	& 95.0	& 63.1	& 97.3	& 95.5	& 89.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using MCD.}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 32.8	& 59.7	& 71.8	& 94.0	& 64.6	\\
mnistm  	& 99.2	& -	& 58.6	& 88.0	& 95.1	& 85.2	\\
svhn    	& 80.2	& 44.2	& -	& 98.8	& 85.9	& 77.3	\\
syndigit	& 91.8	& 51.4	& 88.8	& -	& 88.1	& 80.0	\\
usps    	& 95.5	& 25.3	& 33.4	& 73.3	& -	& 56.9	\\
\midrule
Avg	& 91.7	& 38.4	& 60.1	& 83.0	& 90.8	& 72.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 28.1	& 63.1	& 88.6	& 95.0	& 68.7	\\
mnistm  	& 99.2	& -	& 64.9	& 90.1	& 93.1	& 86.8	\\
svhn    	& 80.7	& 49.6	& -	& 98.9	& 85.3	& 78.6	\\
syndigit	& 92.5	& 62.3	& 89.3	& -	& 86.6	& 82.7	\\
usps    	& 94.2	& 30.4	& 38.2	& 76.7	& -	& 59.9	\\
\midrule
Avg	& 91.6	& 42.6	& 63.9	& 88.6	& 90.0	& 75.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 26.8	& 59.9	& 86.8	& 96.9	& 67.6	\\
mnistm  	& 99.3	& -	& 62.8	& 88.5	& 95.7	& 86.6	\\
svhn    	& 78.5	& 58.0	& -	& 98.9	& 88.8	& 81.0	\\
syndigit	& 92.5	& 70.9	& 89.4	& -	& 87.9	& 85.2	\\
usps    	& 94.2	& 31.8	& 41.4	& 78.6	& -	& 61.5	\\
\midrule
Avg	& 91.1	& 46.9	& 63.4	& 88.2	& 92.3	& 76.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{SSDA DigitFive NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 32.2	& 66.7	& 87.6	& 96.9	& 70.8	\\
mnistm  	& 99.2	& -	& 79.3	& 91.7	& 95.6	& 91.4	\\
svhn    	& 86.6	& 68.9	& -	& 98.8	& 89.2	& 85.9	\\
syndigit	& 93.4	& 75.3	& 90.5	& -	& 89.2	& 87.1	\\
usps    	& 94.9	& 62.7	& 34.0	& 78.0	& -	& 67.4	\\
\midrule
Avg	& 93.5	& 59.8	& 67.6	& 89.0	& 92.7	& 80.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSDA setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 AdaMatch (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 14.7	& 35.0	& 34.5	& 47.3	& 47.0	& 35.7	\\
infograph	& 37.9	& -	& 26.9	& 22.8	& 37.8	& 29.9	& 31.1	\\
painting	& 48.9	& 15.5	& -	& 28.5	& 51.0	& 43.3	& 37.4	\\
quickdraw	& 37.0	& 2.9	& 13.8	& -	& 27.8	& 24.1	& 21.1	\\
real    	& 59.6	& 17.9	& 47.9	& 36.5	& -	& 45.3	& 41.4	\\
sketch  	& 61.5	& 16.4	& 42.2	& 39.0	& 50.4	& -	& 41.9	\\
\midrule
Avg	& 49.0	& 13.5	& 33.2	& 32.3	& 42.9	& 37.9	& 34.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 AdaMatch (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 15.6	& 38.6	& 50.9	& 53.0	& 50.1	& 41.6	\\
infograph	& 48.1	& -	& 32.9	& 43.1	& 46.2	& 39.3	& 41.9	\\
painting	& 55.0	& 16.6	& -	& 44.8	& 56.0	& 48.3	& 44.1	\\
quickdraw	& 51.3	& 6.8	& 26.5	& -	& 43.0	& 36.4	& 32.8	\\
real    	& 65.0	& 19.4	& 49.8	& 51.7	& -	& 50.4	& 47.3	\\
sketch  	& 64.2	& 17.4	& 44.5	& 49.9	& 54.7	& -	& 46.1	\\
\midrule
Avg	& 56.7	& 15.2	& 38.5	& 48.1	& 50.6	& 44.9	& 42.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 AdaMatch (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 17.6	& 41.9	& 55.6	& 57.5	& 53.8	& 45.3	\\
infograph	& 53.2	& -	& 37.2	& 50.3	& 52.5	& 45.2	& 47.7	\\
painting	& 59.4	& 17.8	& -	& 52.6	& 59.9	& 51.2	& 48.2	\\
quickdraw	& 56.7	& 10.0	& 34.6	& -	& 51.0	& 44.5	& 39.4	\\
real    	& 67.6	& 20.9	& 51.8	& 56.9	& -	& 54.3	& 50.3	\\
sketch  	& 66.4	& 19.4	& 47.2	& 55.8	& 58.6	& -	& 49.5	\\
\midrule
Avg	& 60.7	& 17.1	& 42.5	& 54.2	& 55.9	& 49.8	& 46.7 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 AdaMatch (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 20.8	& 49.2	& 62.0	& 64.2	& 58.1	& 50.9	\\
infograph	& 61.5	& -	& 44.9	& 58.4	& 60.9	& 51.5	& 55.4	\\
painting	& 65.3	& 21.0	& -	& 59.5	& 66.2	& 56.9	& 53.8	\\
quickdraw	& 64.1	& 14.8	& 44.5	& -	& 61.1	& 52.6	& 47.4	\\
real    	& 71.1	& 24.2	& 56.1	& 62.9	& -	& 58.6	& 54.6	\\
sketch  	& 70.6	& 22.7	& 52.4	& 61.9	& 64.9	& -	& 54.5	\\
\midrule
Avg	& 66.5	& 20.7	& 49.4	& 60.9	& 63.5	& 55.5	& 52.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 BaselineBN (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.7	& 25.2	& 22.5	& 36.4	& 38.2	& 26.8	\\
infograph	& 24.9	& -	& 17.1	& 14.3	& 24.3	& 20.9	& 20.3	\\
painting	& 39.7	& 12.2	& -	& 17.7	& 44.2	& 34.1	& 29.6	\\
quickdraw	& 24.7	& 2.4	& 7.4	& -	& 15.2	& 15.8	& 13.1	\\
real    	& 47.9	& 14.7	& 40.4	& 20.2	& -	& 35.1	& 31.7	\\
sketch  	& 51.4	& 12.1	& 31.4	& 20.5	& 37.4	& -	& 30.6	\\
\midrule
Avg	& 37.7	& 10.6	& 24.3	& 19.0	& 31.5	& 28.8	& 25.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 BaselineBN (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.8	& 29.8	& 39.8	& 42.9	& 43.2	& 33.7	\\
infograph	& 38.9	& -	& 22.2	& 33.7	& 34.5	& 29.9	& 31.8	\\
painting	& 49.4	& 13.7	& -	& 36.0	& 50.2	& 40.4	& 37.9	\\
quickdraw	& 38.6	& 5.2	& 15.8	& -	& 27.4	& 25.9	& 22.6	\\
real    	& 56.0	& 15.8	& 43.0	& 37.9	& -	& 41.6	& 38.9	\\
sketch  	& 57.6	& 13.8	& 34.7	& 38.5	& 43.6	& -	& 37.6	\\
\midrule
Avg	& 48.1	& 12.3	& 29.1	& 37.2	& 39.7	& 36.2	& 33.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 BaselineBN (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 14.5	& 33.9	& 47.5	& 48.6	& 47.5	& 38.4	\\
infograph	& 47.3	& -	& 27.1	& 43.6	& 41.8	& 36.7	& 39.3	\\
painting	& 55.0	& 15.5	& -	& 45.1	& 54.2	& 45.2	& 43.0	\\
quickdraw	& 46.1	& 7.8	& 21.9	& -	& 37.1	& 33.9	& 29.4	\\
real    	& 59.9	& 18.0	& 45.7	& 46.3	& -	& 46.9	& 43.4	\\
sketch  	& 61.0	& 15.7	& 38.3	& 47.3	& 49.8	& -	& 42.4	\\
\midrule
Avg	& 53.9	& 14.3	& 33.4	& 46.0	& 46.3	& 42.0	& 39.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 BaselineBN (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 18.1	& 43.0	& 56.5	& 57.0	& 53.8	& 45.7	\\
infograph	& 59.5	& -	& 38.3	& 54.0	& 53.8	& 47.7	& 50.7	\\
painting	& 63.5	& 18.9	& -	& 55.3	& 60.9	& 52.5	& 50.2	\\
quickdraw	& 57.3	& 12.9	& 35.2	& -	& 49.6	& 44.8	& 40.0	\\
real    	& 66.3	& 21.3	& 51.2	& 56.0	& -	& 53.9	& 49.7	\\
sketch  	& 67.0	& 20.4	& 46.2	& 56.0	& 57.9	& -	& 49.5	\\
\midrule
Avg	& 62.7	& 18.3	& 42.8	& 55.6	& 55.8	& 50.5	& 47.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.5	& 28.6	& 30.2	& 41.3	& 41.6	& 30.8	\\
infograph	& 27.8	& -	& 17.4	& 17.8	& 25.9	& 22.0	& 22.2	\\
painting	& 43.6	& 12.2	& -	& 23.3	& 45.9	& 35.1	& 32.0	\\
quickdraw	& 35.3	& 2.5	& 10.5	& -	& 19.7	& 18.3	& 17.3	\\
real    	& 51.2	& 14.4	& 40.9	& 25.9	& -	& 37.2	& 33.9	\\
sketch  	& 54.9	& 12.7	& 33.1	& 28.2	& 39.6	& -	& 33.7	\\
\midrule
Avg	& 42.6	& 10.9	& 26.1	& 25.1	& 34.5	& 30.8	& 28.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 13.9	& 35.2	& 48.8	& 49.1	& 48.1	& 39.0	\\
infograph	& 46.5	& -	& 24.5	& 41.7	& 39.0	& 34.3	& 37.2	\\
painting	& 54.7	& 13.7	& -	& 44.6	& 51.9	& 43.4	& 41.7	\\
quickdraw	& 51.2	& 5.7	& 22.8	& -	& 36.8	& 34.1	& 30.1	\\
real    	& 60.4	& 15.6	& 44.4	& 45.9	& -	& 44.4	& 42.1	\\
sketch  	& 61.9	& 14.1	& 38.5	& 47.9	& 48.2	& -	& 42.1	\\
\midrule
Avg	& 54.9	& 12.6	& 33.1	& 45.8	& 45.0	& 40.9	& 38.7 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 16.0	& 40.3	& 55.3	& 54.6	& 51.8	& 43.6	\\
infograph	& 55.1	& -	& 30.7	& 50.5	& 46.6	& 41.5	& 44.9	\\
painting	& 60.3	& 15.4	& -	& 52.6	& 56.4	& 48.6	& 46.7	\\
quickdraw	& 56.5	& 8.9	& 31.1	& -	& 46.1	& 41.4	& 36.8	\\
real    	& 64.2	& 18.0	& 47.0	& 53.3	& -	& 49.6	& 46.4	\\
sketch  	& 64.8	& 16.0	& 42.7	& 54.3	& 54.4	& -	& 46.4	\\
\midrule
Avg	& 60.2	& 14.9	& 38.4	& 53.2	& 51.6	& 46.6	& 44.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 19.2	& 47.9	& 60.8	& 61.6	& 56.7	& 49.2	\\
infograph	& 64.3	& -	& 41.7	& 58.4	& 57.0	& 51.3	& 54.5	\\
painting	& 66.5	& 18.4	& -	& 59.2	& 62.3	& 54.8	& 52.2	\\
quickdraw	& 63.7	& 13.5	& 42.9	& -	& 56.5	& 50.1	& 45.3	\\
real    	& 69.1	& 21.2	& 50.2	& 60.2	& -	& 56.3	& 51.4	\\
sketch  	& 69.2	& 20.1	& 49.8	& 60.5	& 61.4	& -	& 52.2	\\
\midrule
Avg	& 66.6	& 18.5	& 46.5	& 59.8	& 59.8	& 53.8	& 50.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 MCD (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 5.5	& 11.2	& 16.0	& 22.0	& 18.8	& 14.7	\\
infograph	& 9.1	& -	& 6.1	& 7.2	& 9.7	& 4.6	& 7.3	\\
painting	& 20.8	& 5.5	& -	& 9.6	& 27.4	& 13.8	& 15.4	\\
quickdraw	& 8.4	& 1.0	& 1.5	& -	& 3.8	& 4.3	& 3.8	\\
real    	& 35.8	& 9.4	& 27.2	& 12.6	& -	& 19.8	& 21.0	\\
sketch  	& 32.5	& 6.2	& 15.2	& 17.6	& 22.0	& -	& 18.7	\\
\midrule
Avg	& 21.3	& 5.5	& 12.2	& 12.6	& 17.0	& 12.3	& 13.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using MCD.}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 MCD (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 5.8	& 12.4	& 29.2	& 24.6	& 23.0	& 19.0	\\
infograph	& 13.9	& -	& 7.1	& 22.5	& 13.5	& 7.1	& 12.8	\\
painting	& 23.7	& 5.8	& -	& 25.7	& 29.0	& 15.3	& 19.9	\\
quickdraw	& 16.9	& 1.9	& 3.0	& -	& 9.9	& 9.6	& 8.3	\\
real    	& 38.6	& 9.7	& 26.5	& 26.4	& -	& 22.3	& 24.7	\\
sketch  	& 36.3	& 6.1	& 15.6	& 29.0	& 25.0	& -	& 22.4	\\
\midrule
Avg	& 25.9	& 5.9	& 12.9	& 26.6	& 20.4	& 15.5	& 17.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using MCD.}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 MCD (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 7.0	& 14.3	& 37.8	& 30.5	& 28.2	& 23.6	\\
infograph	& 20.8	& -	& 9.2	& 32.0	& 19.2	& 15.5	& 19.3	\\
painting	& 29.3	& 6.8	& -	& 33.2	& 33.3	& 24.1	& 25.3	\\
quickdraw	& 26.0	& 2.9	& 5.8	& -	& 16.8	& 17.6	& 13.8	\\
real    	& 42.9	& 10.8	& 28.9	& 34.5	& -	& 27.8	& 29.0	\\
sketch  	& 42.5	& 7.0	& 17.5	& 38.4	& 31.2	& -	& 27.3	\\
\midrule
Avg	& 32.3	& 6.9	& 15.1	& 35.2	& 26.2	& 22.6	& 23.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using MCD.}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 MCD (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 10.3	& 22.6	& 46.7	& 41.2	& 39.5	& 32.1	\\
infograph	& 34.2	& -	& 16.9	& 43.5	& 30.8	& 29.9	& 31.1	\\
painting	& 42.6	& 8.9	& -	& 45.7	& 42.7	& 37.9	& 35.6	\\
quickdraw	& 40.4	& 5.3	& 15.4	& -	& 30.5	& 30.6	& 24.4	\\
real    	& 50.1	& 12.9	& 34.3	& 46.2	& -	& 38.4	& 36.4	\\
sketch  	& 50.6	& 11.2	& 28.0	& 47.0	& 41.5	& -	& 35.7	\\
\midrule
Avg	& 43.6	& 9.7	& 23.4	& 45.8	& 37.3	& 35.3	& 32.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using MCD.}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.1	& 28.8	& 24.9	& 39.8	& 42.6	& 29.6	\\
infograph	& 27.5	& -	& 19.9	& 8.1	& 25.5	& 22.1	& 20.6	\\
painting	& 40.9	& 11.0	& -	& 9.7	& 43.9	& 33.5	& 27.8	\\
quickdraw	& 25.8	& 2.0	& 6.1	& -	& 12.7	& 15.9	& 12.5	\\
real    	& 48.1	& 13.1	& 41.1	& 14.4	& -	& 34.0	& 30.1	\\
sketch  	& 56.5	& 13.7	& 37.1	& 27.0	& 43.0	& -	& 35.5	\\
\midrule
Avg	& 39.8	& 10.4	& 26.6	& 16.8	& 33.0	& 29.6	& 26.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 13.3	& 31.9	& 36.4	& 44.3	& 45.8	& 34.3	\\
infograph	& 39.7	& -	& 25.4	& 26.5	& 36.0	& 29.9	& 31.5	\\
painting	& 48.7	& 12.9	& -	& 24.5	& 49.9	& 38.0	& 34.8	\\
quickdraw	& 35.1	& 4.3	& 15.0	& -	& 25.8	& 24.2	& 20.9	\\
real    	& 54.8	& 14.4	& 43.5	& 32.7	& -	& 40.6	& 37.2	\\
sketch  	& 59.2	& 14.4	& 39.4	& 37.5	& 46.9	& -	& 39.5	\\
\midrule
Avg	& 47.5	& 11.9	& 31.0	& 31.5	& 40.6	& 35.7	& 33.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 15.3	& 36.5	& 44.4	& 48.5	& 49.2	& 38.8	\\
infograph	& 47.9	& -	& 29.8	& 38.3	& 41.0	& 37.0	& 38.8	\\
painting	& 53.7	& 14.7	& -	& 35.8	& 52.6	& 42.6	& 39.9	\\
quickdraw	& 43.4	& 6.5	& 20.8	& -	& 34.6	& 32.3	& 27.5	\\
real    	& 58.5	& 16.4	& 45.9	& 43.8	& -	& 45.1	& 41.9	\\
sketch  	& 62.1	& 16.9	& 42.1	& 45.2	& 51.7	& -	& 43.6	\\
\midrule
Avg	& 53.1	& 14.0	& 35.0	& 41.5	& 45.7	& 41.2	& 38.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet224 NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 18.8	& 43.0	& 53.0	& 55.3	& 53.7	& 44.8	\\
infograph	& 58.0	& -	& 39.4	& 51.6	& 50.8	& 46.4	& 49.2	\\
painting	& 61.5	& 17.9	& -	& 49.9	& 57.3	& 49.6	& 47.2	\\
quickdraw	& 54.5	& 11.8	& 33.7	& -	& 47.2	& 42.6	& 38.0	\\
real    	& 64.0	& 20.0	& 49.6	& 54.0	& -	& 51.6	& 47.8	\\
sketch  	& 65.9	& 20.3	& 48.4	& 53.8	& 55.7	& -	& 48.8	\\
\midrule
Avg	& 60.8	& 17.8	& 42.8	& 52.5	& 53.3	& 48.8	& 46.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 AdaMatch (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.7	& 28.1	& 37.1	& 40.7	& 39.7	& 31.5	\\
infograph	& 29.2	& -	& 20.5	& 23.3	& 31.0	& 24.1	& 25.6	\\
painting	& 42.8	& 12.6	& -	& 26.5	& 44.7	& 36.4	& 32.6	\\
quickdraw	& 35.7	& 2.6	& 13.2	& -	& 25.1	& 22.2	& 19.8	\\
real    	& 54.6	& 15.3	& 40.7	& 34.0	& -	& 39.2	& 36.8	\\
sketch  	& 54.7	& 13.6	& 34.9	& 35.7	& 43.0	& -	& 36.4	\\
\midrule
Avg	& 43.4	& 11.2	& 27.5	& 31.3	& 36.9	& 32.3	& 30.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 AdaMatch (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.4	& 30.4	& 47.8	& 45.8	& 42.1	& 35.7	\\
infograph	& 40.4	& -	& 24.1	& 39.4	& 38.5	& 29.7	& 34.4	\\
painting	& 48.5	& 12.9	& -	& 41.4	& 48.5	& 39.6	& 38.2	\\
quickdraw	& 46.8	& 5.4	& 21.2	& -	& 37.0	& 30.4	& 28.2	\\
real    	& 58.5	& 15.8	& 42.4	& 49.1	& -	& 43.3	& 41.8	\\
sketch  	& 58.1	& 13.5	& 36.9	& 46.6	& 47.2	& -	& 40.5	\\
\midrule
Avg	& 50.5	& 12.0	& 31.0	& 44.9	& 43.4	& 37.0	& 36.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 AdaMatch (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 13.9	& 34.4	& 52.9	& 49.7	& 45.3	& 39.2	\\
infograph	& 45.9	& -	& 28.3	& 47.6	& 43.3	& 35.8	& 40.2	\\
painting	& 52.8	& 14.3	& -	& 49.0	& 52.0	& 43.2	& 42.3	\\
quickdraw	& 52.0	& 7.2	& 27.3	& -	& 44.3	& 36.8	& 33.5	\\
real    	& 61.2	& 17.5	& 44.7	& 54.9	& -	& 46.5	& 45.0	\\
sketch  	& 60.1	& 15.1	& 39.4	& 52.8	& 50.7	& -	& 43.6	\\
\midrule
Avg	& 54.4	& 13.6	& 34.8	& 51.4	& 48.0	& 41.5	& 40.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 AdaMatch (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 16.8	& 40.7	& 59.0	& 56.5	& 50.3	& 44.7	\\
infograph	& 54.5	& -	& 35.1	& 55.4	& 51.7	& 42.7	& 47.9	\\
painting	& 58.6	& 16.3	& -	& 56.5	& 57.8	& 48.7	& 47.6	\\
quickdraw	& 58.1	& 12.0	& 37.0	& -	& 53.5	& 44.3	& 41.0	\\
real    	& 65.5	& 19.5	& 47.9	& 60.7	& -	& 51.2	& 49.0	\\
sketch  	& 64.0	& 17.6	& 43.8	& 58.9	& 56.6	& -	& 48.2	\\
\midrule
Avg	& 60.1	& 16.4	& 40.9	& 58.1	& 55.2	& 47.4	& 46.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 BaselineBN (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 9.3	& 19.7	& 22.2	& 31.1	& 31.1	& 22.7	\\
infograph	& 18.1	& -	& 11.8	& 11.4	& 17.4	& 14.1	& 14.6	\\
painting	& 31.8	& 9.7	& -	& 15.8	& 37.7	& 25.1	& 24.0	\\
quickdraw	& 22.3	& 2.0	& 5.6	& -	& 13.0	& 13.2	& 11.2	\\
real    	& 42.4	& 12.6	& 34.5	& 19.2	& -	& 29.2	& 27.6	\\
sketch  	& 43.1	& 9.7	& 22.1	& 19.3	& 29.3	& -	& 24.7	\\
\midrule
Avg	& 31.5	& 8.7	& 18.7	& 17.6	& 25.7	& 22.5	& 20.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 BaselineBN (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 10.6	& 23.7	& 37.3	& 37.6	& 35.9	& 29.0	\\
infograph	& 30.2	& -	& 16.2	& 29.0	& 27.1	& 21.7	& 24.8	\\
painting	& 41.5	& 10.6	& -	& 33.5	& 42.5	& 32.6	& 32.1	\\
quickdraw	& 34.5	& 4.2	& 12.4	& -	& 23.9	& 21.6	& 19.3	\\
real    	& 50.1	& 13.4	& 36.9	& 35.6	& -	& 35.5	& 34.3	\\
sketch  	& 49.9	& 10.5	& 26.4	& 36.1	& 36.4	& -	& 31.9	\\
\midrule
Avg	& 41.2	& 9.9	& 23.1	& 34.3	& 33.5	& 29.5	& 28.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 BaselineBN (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.3	& 27.6	& 45.4	& 43.2	& 40.6	& 33.8	\\
infograph	& 39.0	& -	& 20.1	& 39.6	& 34.1	& 28.3	& 32.2	\\
painting	& 48.0	& 12.2	& -	& 42.4	& 46.9	& 37.3	& 37.4	\\
quickdraw	& 42.4	& 6.2	& 17.6	& -	& 32.6	& 27.9	& 25.3	\\
real    	& 54.4	& 15.6	& 39.1	& 44.5	& -	& 40.1	& 38.7	\\
sketch  	& 54.5	& 12.5	& 30.1	& 44.1	& 42.3	& -	& 36.7	\\
\midrule
Avg	& 47.7	& 11.8	& 26.9	& 43.2	& 39.8	& 34.8	& 34.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 BaselineBN (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 15.1	& 36.3	& 54.4	& 51.1	& 46.7	& 40.7	\\
infograph	& 51.9	& -	& 30.6	& 50.2	& 45.5	& 38.4	& 43.3	\\
painting	& 56.6	& 15.0	& -	& 52.9	& 53.8	& 45.0	& 44.7	\\
quickdraw	& 52.2	& 10.3	& 29.2	& -	& 44.5	& 38.6	& 35.0	\\
real    	& 61.5	& 17.8	& 44.0	& 54.1	& -	& 47.1	& 44.9	\\
sketch  	& 60.5	& 15.7	& 38.2	& 53.9	& 51.0	& -	& 43.9	\\
\midrule
Avg	& 56.5	& 14.8	& 35.7	& 53.1	& 49.2	& 43.2	& 42.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.0	& 24.5	& 29.4	& 36.7	& 36.6	& 27.6	\\
infograph	& 22.4	& -	& 13.5	& 14.1	& 21.7	& 17.1	& 17.8	\\
painting	& 37.6	& 10.7	& -	& 20.4	& 40.8	& 29.1	& 27.7	\\
quickdraw	& 31.9	& 2.2	& 7.7	& -	& 16.6	& 16.2	& 14.9	\\
real    	& 47.5	& 13.3	& 37.0	& 24.4	& -	& 32.9	& 31.0	\\
sketch  	& 49.8	& 10.7	& 27.3	& 25.9	& 34.2	& -	& 29.6	\\
\midrule
Avg	& 37.8	& 9.6	& 22.0	& 22.8	& 30.0	& 26.4	& 24.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.3	& 29.9	& 46.5	& 44.8	& 41.4	& 35.0	\\
infograph	& 39.0	& -	& 19.2	& 37.7	& 32.2	& 26.6	& 30.9	\\
painting	& 48.6	& 11.7	& -	& 42.0	& 45.9	& 36.6	& 37.0	\\
quickdraw	& 46.5	& 5.2	& 18.0	& -	& 32.6	& 27.9	& 26.0	\\
real    	& 56.0	& 14.5	& 39.8	& 45.0	& -	& 39.9	& 39.0	\\
sketch  	& 55.9	& 12.0	& 32.2	& 45.0	& 42.3	& -	& 37.5	\\
\midrule
Avg	& 49.2	& 11.1	& 27.8	& 43.2	& 39.6	& 34.5	& 34.2 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 13.9	& 34.9	& 53.3	& 49.9	& 45.3	& 39.5	\\
infograph	& 48.5	& -	& 25.1	& 47.3	& 39.7	& 33.1	& 38.7	\\
painting	& 54.8	& 13.5	& -	& 50.3	& 50.4	& 41.5	& 42.1	\\
quickdraw	& 52.4	& 7.3	& 24.9	& -	& 41.8	& 35.3	& 32.3	\\
real    	& 59.5	& 16.4	& 42.4	& 52.5	& -	& 44.5	& 43.1	\\
sketch  	& 59.5	& 13.9	& 36.2	& 51.7	& 48.2	& -	& 41.9	\\
\midrule
Avg	& 54.9	& 13.0	& 32.7	& 51.0	& 46.0	& 39.9	& 39.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 16.8	& 42.0	& 58.9	& 56.5	& 50.2	& 44.9	\\
infograph	& 57.2	& -	& 35.4	& 56.0	& 49.9	& 42.6	& 48.2	\\
painting	& 60.9	& 16.0	& -	& 57.2	& 56.2	& 48.0	& 47.7	\\
quickdraw	& 58.9	& 11.8	& 36.8	& -	& 52.0	& 44.2	& 40.7	\\
real    	& 64.9	& 18.8	& 47.2	& 58.6	& -	& 50.1	& 47.9	\\
sketch  	& 63.6	& 17.0	& 42.9	& 58.3	& 55.1	& -	& 47.4	\\
\midrule
Avg	& 61.1	& 16.1	& 40.9	& 57.8	& 53.9	& 47.0	& 46.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 MCD (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 6.0	& 12.3	& 15.0	& 23.4	& 21.0	& 15.5	\\
infograph	& 10.2	& -	& 7.2	& 7.0	& 11.2	& 7.1	& 8.5	\\
painting	& 22.8	& 6.3	& -	& 8.3	& 28.7	& 17.1	& 16.6	\\
quickdraw	& 9.5	& 1.1	& 2.1	& -	& 5.1	& 4.9	& 4.5	\\
real    	& 35.4	& 9.2	& 26.4	& 9.8	& -	& 19.5	& 20.1	\\
sketch  	& 31.9	& 6.5	& 15.2	& 13.5	& 21.5	& -	& 17.7	\\
\midrule
Avg	& 22.0	& 5.8	& 12.6	& 10.7	& 18.0	& 13.9	& 13.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using MCD.}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 MCD (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 6.5	& 14.7	& 28.7	& 28.4	& 25.6	& 20.8	\\
infograph	& 17.4	& -	& 8.5	& 19.9	& 16.1	& 11.9	& 14.8	\\
painting	& 28.5	& 7.2	& -	& 23.1	& 31.8	& 22.3	& 22.6	\\
quickdraw	& 20.1	& 2.2	& 5.1	& -	& 12.5	& 12.1	& 10.4	\\
real    	& 39.7	& 9.9	& 27.1	& 24.1	& -	& 24.8	& 25.1	\\
sketch  	& 37.4	& 7.0	& 17.5	& 27.2	& 26.9	& -	& 23.2	\\
\midrule
Avg	& 28.6	& 6.6	& 14.6	& 24.6	& 23.1	& 19.3	& 19.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using MCD.}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 MCD (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 8.2	& 18.6	& 36.5	& 33.5	& 31.3	& 25.6	\\
infograph	& 24.2	& -	& 11.7	& 29.4	& 22.6	& 17.4	& 21.1	\\
painting	& 34.2	& 8.0	& -	& 32.7	& 0	& 27.9	& 20.6	\\
quickdraw	& 27.8	& 3.4	& 8.9	& -	& 20.5	& 18.6	& 15.8	\\
real    	& 43.4	& 11.1	& 29.6	& 33.7	& -	& 30.4	& 29.6	\\
sketch  	& 42.9	& 8.5	& 20.6	& 35.7	& 32.3	& -	& 28.0	\\
\midrule
Avg	& 34.5	& 7.8	& 17.9	& 33.6	& 21.8	& 25.1	& 23.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using MCD.}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 MCD (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.4	& 27.0	& 46.8	& 42.6	& 39.4	& 33.4	\\
infograph	& 37.1	& -	& 19.7	& 41.8	& 33.8	& 29.4	& 32.4	\\
painting	& 44.9	& 10.5	& -	& 44.2	& 43.3	& 36.8	& 35.9	\\
quickdraw	& 41.1	& 6.3	& 18.1	& -	& 32.4	& 29.7	& 25.5	\\
real    	& 49.8	& 13.4	& 34.0	& 45.2	& -	& 38.7	& 36.2	\\
sketch  	& 49.7	& 11.6	& 29.2	& 46.0	& 41.1	& -	& 35.5	\\
\midrule
Avg	& 44.5	& 10.6	& 25.6	& 44.8	& 38.6	& 34.8	& 33.2 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using MCD.}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 10.5	& 23.5	& 22.5	& 35.8	& 36.6	& 25.8	\\
infograph	& 23.9	& -	& 16.2	& 6.7	& 22.9	& 19.1	& 17.8	\\
painting	& 37.5	& 10.8	& -	& 8.8	& 41.8	& 29.8	& 25.7	\\
quickdraw	& 23.3	& 1.5	& 2.6	& -	& 9.5	& 10.9	& 9.6	\\
real    	& 45.2	& 12.3	& 36.3	& 12.6	& -	& 32.0	& 27.7	\\
sketch  	& 51.4	& 11.5	& 28.5	& 23.3	& 36.3	& -	& 30.2	\\
\midrule
Avg	& 36.3	& 9.3	& 21.4	& 14.8	& 29.3	& 25.7	& 22.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.7	& 26.8	& 33.5	& 40.0	& 39.8	& 30.4	\\
infograph	& 33.3	& -	& 20.0	& 19.6	& 30.3	& 24.8	& 25.6	\\
painting	& 44.5	& 11.7	& -	& 21.6	& 45.8	& 34.0	& 31.5	\\
quickdraw	& 31.9	& 3.1	& 5.6	& -	& 16.5	& 18.9	& 15.2	\\
real    	& 50.8	& 13.4	& 39.1	& 30.7	& -	& 37.2	& 34.2	\\
sketch  	& 54.6	& 12.2	& 31.1	& 33.5	& 41.5	& -	& 34.6	\\
\midrule
Avg	& 43.0	& 10.4	& 24.5	& 27.8	& 34.8	& 30.9	& 28.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.9	& 29.6	& 42.6	& 43.8	& 43.0	& 34.4	\\
infograph	& 40.6	& -	& 25.4	& 33.3	& 36.1	& 30.6	& 33.2	\\
painting	& 49.2	& 13.3	& -	& 32.4	& 48.9	& 38.6	& 36.5	\\
quickdraw	& 38.8	& 5.1	& 13.3	& -	& 22.3	& 24.8	& 20.9	\\
real    	& 55.3	& 15.2	& 40.7	& 39.4	& -	& 40.8	& 38.3	\\
sketch  	& 57.9	& 14.0	& 34.6	& 40.8	& 45.4	& -	& 38.5	\\
\midrule
Avg	& 48.4	& 12.1	& 28.7	& 37.7	& 39.3	& 35.6	& 33.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{SSDA DomainNet64 NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 16.1	& 37.1	& 52.3	& 50.3	& 48.2	& 40.8	\\
infograph	& 51.4	& -	& 33.9	& 48.0	& 45.8	& 39.4	& 43.7	\\
painting	& 56.7	& 16.0	& -	& 46.7	& 54.6	& 44.8	& 43.8	\\
quickdraw	& 48.7	& 9.4	& 21.6	& -	& 38.0	& 37.4	& 31.0	\\
real    	& 60.2	& 17.9	& 45.4	& 51.0	& -	& 47.1	& 44.3	\\
sketch  	& 61.8	& 17.3	& 41.6	& 51.6	& 51.7	& -	& 44.8	\\
\midrule
Avg	& 55.8	& 15.3	& 35.9	& 49.9	& 48.1	& 43.4	& 41.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSDA setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive AdaMatch (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 10.1	\\
svhn    	& 39.8	\\
syndigit	& 99.2	\\
usps    	& 96.3	\\
\midrule
Avg	& 68.6	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive AdaMatch (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 98.0	\\
mnistm  	& 97.3	\\
svhn    	& 96.3	\\
syndigit	& 99.1	\\
usps    	& 95.5	\\
\midrule
Avg	& 97.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive AdaMatch (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 97.1	\\
svhn    	& 95.7	\\
syndigit	& 99.4	\\
usps    	& 96.5	\\
\midrule
Avg	& 97.6	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive AdaMatch (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.2	\\
syndigit	& 97.8	\\
usps    	& 97.3	\\
\midrule
Avg	& 97.7	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive BaselineBN (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 64.4	\\
mnistm  	& 14.6	\\
svhn    	& 16.9	\\
syndigit	& 41.0	\\
usps    	& 63.0	\\
\midrule
Avg	& 40.0	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive BaselineBN (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 83.2	\\
mnistm  	& 29.9	\\
svhn    	& 36.5	\\
syndigit	& 77.9	\\
usps    	& 81.9	\\
\midrule
Avg	& 61.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive BaselineBN (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 91.1	\\
mnistm  	& 51.5	\\
svhn    	& 54.0	\\
syndigit	& 83.5	\\
usps    	& 88.5	\\
\midrule
Avg	& 73.7	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive BaselineBN (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 95.3	\\
mnistm  	& 78.3	\\
svhn    	& 69.5	\\
syndigit	& 94.4	\\
usps    	& 94.3	\\
\midrule
Avg	& 86.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 9.9	\\
svhn    	& 31.5	\\
syndigit	& 37.9	\\
usps    	& 80.4	\\
\midrule
Avg	& 51.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 97.4	\\
svhn    	& 82.2	\\
syndigit	& 99.1	\\
usps    	& 97.2	\\
\midrule
Avg	& 94.8	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 99.3	\\
mnistm  	& 98.9	\\
svhn    	& 96.8	\\
syndigit	& 99.5	\\
usps    	& 97.0	\\
\midrule
Avg	& 98.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.9	\\
syndigit	& 99.4	\\
usps    	& 97.2	\\
\midrule
Avg	& 98.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive MCD (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 61.6	\\
mnistm  	& 10.4	\\
svhn    	& 8.5	\\
syndigit	& 9.7	\\
usps    	& 46.8	\\
\midrule
Avg	& 27.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using MCD.}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive MCD (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 90.9	\\
mnistm  	& 18.8	\\
svhn    	& 11.5	\\
syndigit	& 40.5	\\
usps    	& 92.5	\\
\midrule
Avg	& 50.8	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using MCD.}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive MCD (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 94.8	\\
mnistm  	& 80.4	\\
svhn    	& 31.4	\\
syndigit	& 92.4	\\
usps    	& 92.8	\\
\midrule
Avg	& 78.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using MCD.}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive MCD (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 97.1	\\
mnistm  	& 94.4	\\
svhn    	& 82.3	\\
syndigit	& 96.6	\\
usps    	& 94.6	\\
\midrule
Avg	& 93.0	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using MCD.}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 71.2	\\
mnistm  	& 13.1	\\
svhn    	& 16.2	\\
syndigit	& 40.8	\\
usps    	& 75.0	\\
\midrule
Avg	& 43.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 91.0	\\
mnistm  	& 29.6	\\
svhn    	& 41.9	\\
syndigit	& 84.5	\\
usps    	& 89.7	\\
\midrule
Avg	& 67.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 96.8	\\
mnistm  	& 59.9	\\
svhn    	& 62.0	\\
syndigit	& 90.9	\\
usps    	& 92.9	\\
\midrule
Avg	& 80.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DigitFive NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 90.5	\\
svhn    	& 80.0	\\
syndigit	& 95.9	\\
usps    	& 96.3	\\
\midrule
Avg	& 92.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the SSL setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 AdaMatch (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 10.5	\\
infograph	& 1.5	\\
painting	& 3.9	\\
quickdraw	& 18.7	\\
real    	& 8.3	\\
sketch  	& 6.5	\\
\midrule
Avg	& 8.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 AdaMatch (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 41.5	\\
infograph	& 4.0	\\
painting	& 13.0	\\
quickdraw	& 42.0	\\
real    	& 28.6	\\
sketch  	& 25.1	\\
\midrule
Avg	& 25.7	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 AdaMatch (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 51.8	\\
infograph	& 5.8	\\
painting	& 21.7	\\
quickdraw	& 51.5	\\
real    	& 42.4	\\
sketch  	& 36.5	\\
\midrule
Avg	& 35.0	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 AdaMatch (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 62.6	\\
infograph	& 10.3	\\
painting	& 39.5	\\
quickdraw	& 59.8	\\
real    	& 56.5	\\
sketch  	& 49.6	\\
\midrule
Avg	& 46.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 BaselineBN (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 7.4	\\
infograph	& 1.3	\\
painting	& 3.4	\\
quickdraw	& 14.5	\\
real    	& 7.0	\\
sketch  	& 5.3	\\
\midrule
Avg	& 6.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 BaselineBN (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 26.6	\\
infograph	& 3.3	\\
painting	& 9.1	\\
quickdraw	& 33.1	\\
real    	& 20.1	\\
sketch  	& 16.6	\\
\midrule
Avg	& 18.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 BaselineBN (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 37.9	\\
infograph	& 5.0	\\
painting	& 13.5	\\
quickdraw	& 42.6	\\
real    	& 31.1	\\
sketch  	& 26.9	\\
\midrule
Avg	& 26.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 BaselineBN (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 53.2	\\
infograph	& 8.2	\\
painting	& 28.0	\\
quickdraw	& 53.8	\\
real    	& 46.2	\\
sketch  	& 41.4	\\
\midrule
Avg	& 38.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 9.3	\\
infograph	& 1.4	\\
painting	& 3.6	\\
quickdraw	& 17.8	\\
real    	& 7.6	\\
sketch  	& 6.1	\\
\midrule
Avg	& 7.6	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 40.2	\\
infograph	& 3.5	\\
painting	& 10.5	\\
quickdraw	& 41.6	\\
real    	& 26.7	\\
sketch  	& 22.7	\\
\midrule
Avg	& 24.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 50.6	\\
infograph	& 5.1	\\
painting	& 15.7	\\
quickdraw	& 50.7	\\
real    	& 38.4	\\
sketch  	& 33.5	\\
\midrule
Avg	& 32.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 60.5	\\
infograph	& 8.5	\\
painting	& 32.2	\\
quickdraw	& 58.3	\\
real    	& 51.2	\\
sketch  	& 46.5	\\
\midrule
Avg	& 42.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 MCD (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 2.3	\\
infograph	& 0.9	\\
painting	& 1.7	\\
quickdraw	& 7.5	\\
real    	& 3.0	\\
sketch  	& 1.2	\\
\midrule
Avg	& 2.8	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using MCD.}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 MCD (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 9.2	\\
infograph	& 1.9	\\
painting	& 3.8	\\
quickdraw	& 25.1	\\
real    	& 9.3	\\
sketch  	& 4.0	\\
\midrule
Avg	& 8.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using MCD.}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 MCD (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 16.4	\\
infograph	& 3.4	\\
painting	& 7.1	\\
quickdraw	& 35.7	\\
real    	& 16.2	\\
sketch  	& 10.6	\\
\midrule
Avg	& 14.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using MCD.}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 MCD (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 31.8	\\
infograph	& 5.7	\\
painting	& 15.1	\\
quickdraw	& 47.4	\\
real    	& 28.8	\\
sketch  	& 27.2	\\
\midrule
Avg	& 26.0	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using MCD.}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 9.8	\\
infograph	& 1.5	\\
painting	& 4.0	\\
quickdraw	& 17.5	\\
real    	& 8.6	\\
sketch  	& 7.1	\\
\midrule
Avg	& 8.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 36.4	\\
infograph	& 3.9	\\
painting	& 13.6	\\
quickdraw	& 39.8	\\
real    	& 27.8	\\
sketch  	& 24.0	\\
\midrule
Avg	& 24.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 48.3	\\
infograph	& 5.6	\\
painting	& 20.9	\\
quickdraw	& 49.6	\\
real    	& 41.5	\\
sketch  	& 35.4	\\
\midrule
Avg	& 33.6	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet224 NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 60.8	\\
infograph	& 9.7	\\
painting	& 38.8	\\
quickdraw	& 59.4	\\
real    	& 55.2	\\
sketch  	& 48.5	\\
\midrule
Avg	& 45.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 AdaMatch (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 10.2	\\
infograph	& 1.5	\\
painting	& 4.0	\\
quickdraw	& 18.9	\\
real    	& 8.5	\\
sketch  	& 5.6	\\
\midrule
Avg	& 8.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 AdaMatch (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 36.5	\\
infograph	& 3.6	\\
painting	& 13.3	\\
quickdraw	& 41.7	\\
real    	& 26.9	\\
sketch  	& 21.0	\\
\midrule
Avg	& 23.8	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 AdaMatch (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 46.4	\\
infograph	& 5.8	\\
painting	& 20.8	\\
quickdraw	& 49.9	\\
real    	& 37.9	\\
sketch  	& 29.6	\\
\midrule
Avg	& 31.7	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 AdaMatch (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 56.2	\\
infograph	& 9.3	\\
painting	& 33.3	\\
quickdraw	& 57.7	\\
real    	& 50.3	\\
sketch  	& 41.4	\\
\midrule
Avg	& 41.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 BaselineBN (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 6.9	\\
infograph	& 1.4	\\
painting	& 3.1	\\
quickdraw	& 13.2	\\
real    	& 6.6	\\
sketch  	& 4.3	\\
\midrule
Avg	& 5.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 BaselineBN (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 23.6	\\
infograph	& 3.2	\\
painting	& 9.1	\\
quickdraw	& 31.2	\\
real    	& 18.2	\\
sketch  	& 13.9	\\
\midrule
Avg	& 16.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 BaselineBN (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 33.9	\\
infograph	& 4.8	\\
painting	& 14.2	\\
quickdraw	& 40.3	\\
real    	& 28.2	\\
sketch  	& 22.1	\\
\midrule
Avg	& 23.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 BaselineBN (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 48.2	\\
infograph	& 7.8	\\
painting	& 25.7	\\
quickdraw	& 51.1	\\
real    	& 41.5	\\
sketch  	& 34.9	\\
\midrule
Avg	& 34.9	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 FixMatch+ (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 9.7	\\
infograph	& 1.4	\\
painting	& 3.9	\\
quickdraw	& 17.1	\\
real    	& 7.5	\\
sketch  	& 6.0	\\
\midrule
Avg	& 7.6	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 FixMatch+ (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 37.6	\\
infograph	& 3.5	\\
painting	& 13.1	\\
quickdraw	& 42.3	\\
real    	& 27.2	\\
sketch  	& 21.1	\\
\midrule
Avg	& 24.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 FixMatch+ (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 48.1	\\
infograph	& 5.3	\\
painting	& 18.9	\\
quickdraw	& 50.9	\\
real    	& 39.0	\\
sketch  	& 30.6	\\
\midrule
Avg	& 32.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 FixMatch+ (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 57.2	\\
infograph	& 8.8	\\
painting	& 32.7	\\
quickdraw	& 58.0	\\
real    	& 50.5	\\
sketch  	& 41.6	\\
\midrule
Avg	& 41.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 MCD (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 3.0	\\
infograph	& 1.0	\\
painting	& 1.8	\\
quickdraw	& 7.8	\\
real    	& 3.5	\\
sketch  	& 1.6	\\
\midrule
Avg	& 3.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using MCD.}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 MCD (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 10.5	\\
infograph	& 2.3	\\
painting	& 5.0	\\
quickdraw	& 25.1	\\
real    	& 11.3	\\
sketch  	& 6.9	\\
\midrule
Avg	& 10.2	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using MCD.}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 MCD (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 19.6	\\
infograph	& 3.5	\\
painting	& 9.5	\\
quickdraw	& 35.1	\\
real    	& 18.7	\\
sketch  	& 13.6	\\
\midrule
Avg	& 16.7	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using MCD.}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 MCD (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 34.7	\\
infograph	& 5.6	\\
painting	& 17.3	\\
quickdraw	& 47.1	\\
real    	& 32.3	\\
sketch  	& 27.9	\\
\midrule
Avg	& 27.5	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using MCD.}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '1'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 NoisyStudent (num\_target\_labels=1)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 8.7	\\
infograph	& 1.5	\\
painting	& 4.1	\\
quickdraw	& 16.7	\\
real    	& 7.6	\\
sketch  	& 5.4	\\
\midrule
Avg	& 7.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '5'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 NoisyStudent (num\_target\_labels=5)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 31.8	\\
infograph	& 3.5	\\
painting	& 11.8	\\
quickdraw	& 37.1	\\
real    	& 24.3	\\
sketch  	& 17.9	\\
\midrule
Avg	& 21.1	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '10'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 NoisyStudent (num\_target\_labels=10)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 42.3	\\
infograph	& 5.3	\\
painting	& 18.6	\\
quickdraw	& 46.7	\\
real    	& 35.6	\\
sketch  	& 27.2	\\
\midrule
Avg	& 29.3	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent', 'num_labels': '25'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|r}
\toprule
\multicolumn{2}{c} {\textbf{SSL DomainNet64 NoisyStudent (num\_target\_labels=25)}} \\
\midrule
& Accuracy	\\
\midrule
clipart 	& 54.6	\\
infograph	& 8.7	\\
painting	& 31.7	\\
quickdraw	& 57.4	\\
real    	& 49.4	\\
sketch  	& 40.3	\\
\midrule
Avg	& 40.4	\\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the SSL setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'AdaMatch'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{UDA DigitFive AdaMatch }} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 96.9	& 99.7	& 97.8	& 98.4	\\
mnistm  	& 99.4	& -	& 96.9	& 99.7	& 97.8	& 98.5	\\
svhn    	& 99.3	& 98.9	& -	& 99.6	& 90.4	& 97.0	\\
syndigit	& 99.4	& 99.0	& 97.0	& -	& 95.8	& 97.8	\\
usps    	& 99.3	& 98.9	& 96.6	& 94.9	& -	& 97.4	\\
\midrule
Avg	& 99.4	& 99.0	& 96.8	& 98.5	& 95.5	& 97.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the UDA setting using AdaMatch.}
\label{ tab:da_digitfive32_AdaMatch_None }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'Baseline'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{UDA DigitFive BaselineBN }} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 54.3	& 55.0	& 76.0	& 96.3	& 70.4	\\
mnistm  	& 96.5	& -	& 52.4	& 81.8	& 88.1	& 79.7	\\
svhn    	& 40.4	& 32.0	& -	& 86.3	& 39.9	& 49.6	\\
syndigit	& 67.7	& 30.0	& 79.7	& -	& 70.5	& 62.0	\\
usps    	& 78.6	& 27.3	& 31.9	& 64.8	& -	& 50.6	\\
\midrule
Avg	& 70.8	& 35.9	& 54.8	& 77.2	& 73.7	& 62.5 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the UDA setting using BaselineBN.}
\label{ tab:da_digitfive32_Baseline_None }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'FixMatchDA'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{UDA DigitFive FixMatch+ }} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 99.2	& 97.0	& 99.7	& 97.9	& 98.4	\\
mnistm  	& 99.4	& -	& 97.0	& 99.6	& 85.1	& 95.3	\\
svhn    	& 99.2	& 98.9	& -	& 99.5	& 87.3	& 96.2	\\
syndigit	& 99.3	& 99.0	& 96.9	& -	& 97.2	& 98.1	\\
usps    	& 99.3	& 99.0	& 62.6	& 99.8	& -	& 90.2	\\
\midrule
Avg	& 99.3	& 99.0	& 88.4	& 99.7	& 91.9	& 95.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the UDA setting using FixMatch+.}
\label{ tab:da_digitfive32_FixMatchDA_None }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'MCD'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{UDA DigitFive MCD }} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 10.7	& 13.3	& 11.1	& 90.0	& 31.3	\\
mnistm  	& 92.2	& -	& 13.7	& 13.2	& 52.0	& 42.8	\\
svhn    	& 97.0	& 53.3	& -	& 97.9	& 90.4	& 84.7	\\
syndigit	& 98.3	& 27.9	& 66.0	& -	& 91.7	& 71.0	\\
usps    	& 98.1	& 10.0	& 6.4	& 9.8	& -	& 31.1	\\
\midrule
Avg	& 96.4	& 25.5	& 24.9	& 33.0	& 81.0	& 52.1 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the UDA setting using MCD.}
\label{ tab:da_digitfive32_MCD_None }
\end{table}

%% run {'dataset': 'digitfive32', 'algorithm': 'NoisyStudent'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrr|r}
\toprule
\multicolumn{6}{c} {\textbf{UDA DigitFive NoisyStudent }} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	& Avg\\
\midrule
mnist   	& -	& 30.4	& 51.4	& 81.8	& 97.2	& 65.2	\\
mnistm  	& 99.2	& -	& 63.0	& 89.0	& 97.0	& 87.0	\\
svhn    	& 82.8	& 45.2	& -	& 98.9	& 83.9	& 77.7	\\
syndigit	& 92.6	& 50.5	& 90.0	& -	& 87.1	& 80.0	\\
usps    	& 95.5	& 25.2	& 30.0	& 75.3	& -	& 56.5	\\
\midrule
Avg	& 92.5	& 37.8	& 58.6	& 86.3	& 91.3	& 73.3 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DigitFive in the UDA setting using NoisyStudent.}
\label{ tab:da_digitfive32_NoisyStudent_None }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'AdaMatch'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet224 AdaMatch }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 14.8	& 35.3	& 26.8	& 46.5	& 46.5	& 34.0	\\
infograph	& 21.7	& -	& 11.7	& 0.3	& 20.0	& 0.2	& 10.8	\\
painting	& 45.3	& 13.5	& -	& 13.2	& 48.1	& 41.0	& 32.2	\\
quickdraw	& 33.6	& 2.4	& 10.1	& -	& 19.1	& 21.1	& 17.3	\\
real    	& 56.0	& 16.6	& 47.6	& 22.9	& -	& 42.4	& 37.1	\\
sketch  	& 60.2	& 17.0	& 42.9	& 34.2	& 49.1	& -	& 40.7	\\
\midrule
Avg	& 43.4	& 12.9	& 29.5	& 19.5	& 36.6	& 30.2	& 28.7 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the UDA setting using AdaMatch.}
\label{ tab:da_domainnet224_AdaMatch_None }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'Baseline'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet224 BaselineBN }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.4	& 23.4	& 12.1	& 33.4	& 34.9	& 23.0	\\
infograph	& 16.2	& -	& 13.8	& 0.9	& 16.5	& 11.5	& 11.8	\\
painting	& 33.6	& 11.2	& -	& 1.0	& 41.2	& 25.7	& 22.5	\\
quickdraw	& 11.2	& 0.8	& 2.5	& -	& 5.5	& 7.1	& 5.4	\\
real    	& 43.4	& 13.7	& 39.4	& 2.1	& -	& 29.6	& 25.6	\\
sketch  	& 47.9	& 11.0	& 28.7	& 3.8	& 33.1	& -	& 24.9	\\
\midrule
Avg	& 30.5	& 9.6	& 21.6	& 4.0	& 25.9	& 21.8	& 18.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the UDA setting using BaselineBN.}
\label{ tab:da_domainnet224_Baseline_None }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'FixMatchDA'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet224 FixMatch+ }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 11.6	& 26.4	& 11.2	& 37.6	& 37.8	& 24.9	\\
infograph	& 15.8	& -	& 6.5	& 0.6	& 8.6	& 11.4	& 8.6	\\
painting	& 39.0	& 11.6	& -	& 4.2	& 42.7	& 31.4	& 25.8	\\
quickdraw	& 15.8	& 1.3	& 5.0	& -	& 11.5	& 12.2	& 9.2	\\
real    	& 48.1	& 13.8	& 39.8	& 7.3	& -	& 33.4	& 28.5	\\
sketch  	& 50.3	& 11.8	& 30.7	& 11.8	& 34.2	& -	& 27.8	\\
\midrule
Avg	& 33.8	& 10.0	& 21.7	& 7.0	& 26.9	& 25.2	& 20.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the UDA setting using FixMatch+.}
\label{ tab:da_domainnet224_FixMatchDA_None }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'MCD'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet224 MCD }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 7.7	& 15.2	& 15.2	& 25.8	& 23.4	& 17.5	\\
infograph	& 9.2	& -	& 7.0	& 1.6	& 11.2	& 6.5	& 7.1	\\
painting	& 25.6	& 7.0	& -	& 5.3	& 32.1	& 18.8	& 17.8	\\
quickdraw	& 7.4	& 0.7	& 0.7	& -	& 1.6	& 4.1	& 2.9	\\
real    	& 38.4	& 10.5	& 32.4	& 7.7	& -	& 22.9	& 22.4	\\
sketch  	& 37.2	& 8.2	& 22.9	& 14.7	& 26.7	& -	& 21.9	\\
\midrule
Avg	& 23.6	& 6.8	& 15.6	& 8.9	& 19.5	& 15.1	& 14.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the UDA setting using MCD.}
\label{ tab:da_domainnet224_MCD_None }
\end{table}

%% run {'dataset': 'domainnet224', 'algorithm': 'NoisyStudent'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet224 NoisyStudent }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.9	& 28.5	& 20.4	& 39.5	& 42.3	& 28.7	\\
infograph	& 24.5	& -	& 18.9	& 3.1	& 23.9	& 18.3	& 17.7	\\
painting	& 37.6	& 11.4	& -	& 3.4	& 40.9	& 30.9	& 24.8	\\
quickdraw	& 20.9	& 1.0	& 2.7	& -	& 8.7	& 13.2	& 9.3	\\
real    	& 47.8	& 13.7	& 39.8	& 7.7	& -	& 32.6	& 28.3	\\
sketch  	& 55.2	& 14.8	& 37.1	& 22.8	& 41.8	& -	& 34.3	\\
\midrule
Avg	& 37.2	& 10.8	& 25.4	& 11.5	& 31.0	& 27.5	& 23.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet224 in the UDA setting using NoisyStudent.}
\label{ tab:da_domainnet224_NoisyStudent_None }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'AdaMatch'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet64 AdaMatch }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 12.2	& 29.1	& 27.7	& 40.9	& 40.8	& 30.1	\\
infograph	& 22.3	& -	& 18.2	& 5.4	& 24.7	& 19.9	& 18.1	\\
painting	& 39.7	& 11.7	& -	& 12.6	& 43.4	& 34.9	& 28.5	\\
quickdraw	& 24.6	& 2.4	& 8.4	& -	& 16.4	& 15.5	& 13.5	\\
real    	& 52.2	& 15.0	& 41.6	& 13.3	& -	& 38.6	& 32.1	\\
sketch  	& 53.4	& 13.6	& 35.6	& 25.4	& 41.5	& -	& 33.9	\\
\midrule
Avg	& 38.4	& 11.0	& 26.6	& 16.9	& 33.4	& 29.9	& 26.0 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the UDA setting using AdaMatch.}
\label{ tab:da_domainnet64_AdaMatch_None }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'Baseline'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet64 BaselineBN }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 9.5	& 19.0	& 6.3	& 29.4	& 29.9	& 18.8	\\
infograph	& 12.9	& -	& 10.8	& 0.6	& 14.0	& 9.5	& 9.6	\\
painting	& 27.3	& 9.3	& -	& 1.0	& 36.3	& 21.8	& 19.1	\\
quickdraw	& 10.3	& 0.8	& 1.9	& -	& 4.8	& 5.9	& 4.7	\\
real    	& 39.3	& 11.9	& 34.6	& 2.2	& -	& 25.5	& 22.7	\\
sketch  	& 40.9	& 8.5	& 20.4	& 3.3	& 26.0	& -	& 19.8	\\
\midrule
Avg	& 26.1	& 8.0	& 17.3	& 2.7	& 22.1	& 18.5	& 15.8 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the UDA setting using BaselineBN.}
\label{ tab:da_domainnet64_Baseline_None }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'FixMatchDA'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet64 FixMatch+ }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 10.2	& 24.6	& 14.6	& 35.7	& 35.3	& 24.1	\\
infograph	& 17.9	& -	& 14.3	& 2.2	& 18.7	& 14.2	& 13.5	\\
painting	& 34.7	& 10.7	& -	& 4.2	& 39.7	& 27.7	& 23.4	\\
quickdraw	& 23.7	& 1.4	& 5.1	& -	& 11.2	& 10.2	& 10.3	\\
real    	& 45.4	& 13.5	& 37.4	& 6.6	& -	& 30.7	& 26.7	\\
sketch  	& 48.1	& 10.3	& 26.6	& 10.4	& 31.5	& -	& 25.4	\\
\midrule
Avg	& 34.0	& 9.2	& 21.6	& 7.6	& 27.4	& 23.6	& 20.6 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the UDA setting using FixMatch+.}
\label{ tab:da_domainnet64_FixMatchDA_None }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'MCD'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet64 MCD }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 7.5	& 15.9	& 12.9	& 26.2	& 25.6	& 17.6	\\
infograph	& 11.3	& -	& 9.4	& 2.3	& 13.3	& 8.6	& 9.0	\\
painting	& 25.8	& 7.5	& -	& 4.3	& 32.1	& 21.4	& 18.2	\\
quickdraw	& 8.0	& 0.6	& 0.6	& -	& 1.6	& 4.6	& 3.1	\\
real    	& 37.2	& 10.1	& 29.8	& 6.8	& -	& 22.9	& 21.4	\\
sketch  	& 37.3	& 7.8	& 20.2	& 11.6	& 25.0	& -	& 20.4	\\
\midrule
Avg	& 23.9	& 6.7	& 15.2	& 7.6	& 19.6	& 16.6	& 14.9 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the UDA setting using MCD.}
\label{ tab:da_domainnet64_MCD_None }
\end{table}

%% run {'dataset': 'domainnet64', 'algorithm': 'NoisyStudent'}
\begin{table}[ht!] % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr|r}
\toprule
\multicolumn{7}{c} {\textbf{UDA DomainNet64 NoisyStudent }} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	& Avg\\
\midrule
clipart 	& -	& 10.9	& 24.3	& 18.9	& 35.4	& 36.8	& 25.3	\\
infograph	& 21.2	& -	& 16.9	& 2.6	& 21.8	& 16.0	& 15.7	\\
painting	& 36.1	& 11.7	& -	& 3.6	& 41.5	& 28.5	& 24.3	\\
quickdraw	& 19.0	& 0.9	& 1.5	& -	& 6.8	& 7.2	& 7.1	\\
real    	& 44.0	& 13.8	& 38.3	& 6.6	& -	& 30.6	& 26.7	\\
sketch  	& 50.0	& 12.0	& 30.4	& 18.2	& 36.0	& -	& 29.3	\\
\midrule
Avg	& 34.1	& 9.9	& 22.3	& 10.0	& 28.3	& 23.8	& 21.4 \\
\bottomrule
\end{tabular}
\caption{Individual results for each dataset pair for DomainNet64 in the UDA setting using NoisyStudent.}
\label{ tab:da_domainnet64_NoisyStudent_None }
\end{table}



==> AdaMatch - ICLR 2022/new_autogenerated.tex <==
%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.8	& 97.7	\\
mnistm  	& 96.5	\\
svhn    	& 99.2	\\
syndigit	& 96.9	\\
usps    	& 99.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.1	& 96.6	& 97.8	\\
mnistm  	& 96.7	\\
svhn    	& 99.2	\\
syndigit	& 96.8	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.7	& 97.9	\\
mnistm  	& 96.7	\\
svhn    	& 99.3	\\
syndigit	& 96.7	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.1	& 96.1	& 97.7	\\
mnistm  	& 96.3	\\
svhn    	& 99.3	\\
syndigit	& 96.3	\\
usps    	& 99.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 72.4	& 42.0	& 95.8	\\
mnistm  	& 63.6	\\
svhn    	& 79.8	\\
syndigit	& 76.2	\\
usps    	& 83.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 81.0	& 59.3	& 96.2	\\
mnistm  	& 68.5	\\
svhn    	& 90.5	\\
syndigit	& 80.8	\\
usps    	& 90.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 86.3	& 68.2	& 96.5	\\
mnistm  	& 74.7	\\
svhn    	& 94.7	\\
syndigit	& 84.5	\\
usps    	& 95.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 92.7	& 77.4	& 97.0	\\
mnistm  	& 78.7	\\
svhn    	& 96.8	\\
syndigit	& 86.2	\\
usps    	& 96.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 58.6	& 97.9	\\
mnistm  	& 31.9	\\
svhn    	& 97.9	\\
syndigit	& 97.0	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.9	& 97.8	\\
mnistm  	& 96.9	\\
svhn    	& 97.9	\\
syndigit	& 96.8	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.8	& 98.1	\\
mnistm  	& 96.9	\\
svhn    	& 99.3	\\
syndigit	& 97.0	\\
usps    	& 99.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.5	& 97.9	\\
mnistm  	& 96.5	\\
svhn    	& 99.2	\\
syndigit	& 96.6	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 32.8	& 59.7	& 71.8	& 94.0	\\
mnistm  	& 99.2	& -	& 58.6	& 88.0	& 95.1	\\
svhn    	& 80.2	& 44.2	& -	& 98.8	& 85.9	\\
syndigit	& 91.8	& 51.4	& 88.8	& -	& 88.1	\\
usps    	& 95.5	& 25.3	& 33.4	& 73.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 28.1	& 63.1	& 88.6	& 95.0	\\
mnistm  	& 99.2	& -	& 64.9	& 90.1	& 93.1	\\
svhn    	& 80.7	& 49.6	& -	& 98.9	& 85.3	\\
syndigit	& 92.5	& 62.3	& 89.3	& -	& 86.6	\\
usps    	& 94.2	& 30.4	& 38.2	& 76.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 26.8	& 59.9	& 86.8	& 96.9	\\
mnistm  	& 99.3	& -	& 62.8	& 88.5	& 95.7	\\
svhn    	& 78.5	& 58.0	& -	& 98.9	& 88.8	\\
syndigit	& 92.5	& 70.9	& 89.4	& -	& 87.9	\\
usps    	& 94.2	& 31.8	& 41.4	& 78.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 32.2	& 66.7	& 87.6	& 96.9	\\
mnistm  	& 99.2	& -	& 79.3	& 91.7	& 95.6	\\
svhn    	& 86.6	& 68.9	& -	& 98.8	& 89.2	\\
syndigit	& 93.4	& 75.3	& 90.5	& -	& 89.2	\\
usps    	& 94.9	& 62.7	& 34.0	& 78.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 28.1	& 37.1	& 40.7	& 39.7	\\
infograph	& 29.2	& -	& 20.5	& 23.3	& 31.0	& 24.1	\\
painting	& 42.8	& 12.6	& -	& 26.5	& 44.7	& 36.4	\\
quickdraw	& 35.7	& 2.6	& 13.2	& -	& 25.1	& 22.2	\\
real    	& 54.6	& 15.3	& 40.7	& 34.0	& -	& 39.2	\\
sketch  	& 54.7	& 13.6	& 34.9	& 35.7	& 43.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.4	& 30.4	& 47.8	& 45.8	& 42.1	\\
infograph	& 40.4	& -	& 24.1	& 39.4	& 38.5	& 29.7	\\
painting	& 48.5	& 12.9	& -	& 41.4	& 48.5	& 39.6	\\
quickdraw	& 46.8	& 5.4	& 21.2	& -	& 37.0	& 30.4	\\
real    	& 58.5	& 15.8	& 42.4	& 49.1	& -	& 43.3	\\
sketch  	& 58.1	& 13.5	& 36.9	& 46.6	& 47.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.9	& 34.4	& 52.9	& 49.7	& 45.3	\\
infograph	& 45.9	& -	& 28.3	& 47.6	& 43.3	& 35.8	\\
painting	& 52.8	& 14.3	& -	& 49.0	& 52.0	& 43.2	\\
quickdraw	& 52.0	& 7.2	& 27.3	& -	& 44.3	& 36.8	\\
real    	& 61.2	& 17.5	& 44.7	& 54.9	& -	& 46.5	\\
sketch  	& 60.1	& 15.1	& 39.4	& 52.8	& 50.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.8	& 40.7	& 59.0	& 56.5	& 50.3	\\
infograph	& 54.5	& -	& 35.1	& 55.4	& 51.7	& 42.7	\\
painting	& 58.6	& 16.3	& -	& 56.5	& 57.8	& 48.7	\\
quickdraw	& 58.1	& 12.0	& 37.0	& -	& 53.5	& 44.3	\\
real    	& 65.5	& 19.5	& 47.9	& 60.7	& -	& 51.2	\\
sketch  	& 64.0	& 17.6	& 43.8	& 58.9	& 56.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.3	& 19.7	& 22.2	& 31.1	& 31.1	\\
infograph	& 18.1	& -	& 11.8	& 11.4	& 17.4	& 14.1	\\
painting	& 31.8	& 9.7	& -	& 15.8	& 37.7	& 25.1	\\
quickdraw	& 22.3	& 2.0	& 5.6	& -	& 13.0	& 13.2	\\
real    	& 42.4	& 12.6	& 34.5	& 19.2	& -	& 29.2	\\
sketch  	& 43.1	& 9.7	& 22.1	& 19.3	& 29.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.6	& 23.7	& 37.3	& 37.6	& 35.9	\\
infograph	& 30.2	& -	& 16.2	& 29.0	& 27.1	& 21.7	\\
painting	& 41.5	& 10.6	& -	& 33.5	& 42.5	& 32.6	\\
quickdraw	& 34.5	& 4.2	& 12.4	& -	& 23.9	& 21.6	\\
real    	& 50.1	& 13.4	& 36.9	& 35.6	& -	& 35.5	\\
sketch  	& 49.9	& 10.5	& 26.4	& 36.1	& 36.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.3	& 27.6	& 45.4	& 43.2	& 40.6	\\
infograph	& 39.0	& -	& 20.1	& 39.6	& 34.1	& 28.3	\\
painting	& 48.0	& 12.2	& -	& 42.4	& 46.9	& 37.3	\\
quickdraw	& 42.4	& 6.2	& 17.6	& -	& 32.6	& 27.9	\\
real    	& 54.4	& 15.6	& 39.1	& 44.5	& -	& 40.1	\\
sketch  	& 54.5	& 12.5	& 30.1	& 44.1	& 42.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 15.1	& 36.3	& 54.4	& 51.1	& 46.7	\\
infograph	& 51.9	& -	& 30.6	& 50.2	& 45.5	& 38.4	\\
painting	& 56.6	& 15.0	& -	& 52.9	& 53.8	& 45.0	\\
quickdraw	& 52.2	& 10.3	& 29.2	& -	& 44.5	& 38.6	\\
real    	& 61.5	& 17.8	& 44.0	& 54.1	& -	& 47.1	\\
sketch  	& 60.5	& 15.7	& 38.2	& 53.9	& 51.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.0	& 24.5	& 29.4	& 36.7	& 36.6	\\
infograph	& 22.4	& -	& 13.5	& 14.1	& 21.7	& 17.1	\\
painting	& 37.6	& 10.7	& -	& 20.4	& 40.8	& 29.1	\\
quickdraw	& 31.9	& 2.2	& 7.7	& -	& 16.6	& 16.2	\\
real    	& 47.5	& 13.3	& 37.0	& 24.4	& -	& 32.9	\\
sketch  	& 49.8	& 10.7	& 27.3	& 25.9	& 34.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.3	& 29.9	& 46.5	& 44.8	& 41.4	\\
infograph	& 39.0	& -	& 19.2	& 37.7	& 32.2	& 26.6	\\
painting	& 48.6	& 11.7	& -	& 42.0	& 45.9	& 36.6	\\
quickdraw	& 46.5	& 5.2	& 18.0	& -	& 32.6	& 27.9	\\
real    	& 56.0	& 14.5	& 39.8	& 45.0	& -	& 39.9	\\
sketch  	& 55.9	& 12.0	& 32.2	& 45.0	& 42.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.9	& 34.9	& 53.3	& 49.9	& 45.3	\\
infograph	& 48.5	& -	& 25.1	& 47.3	& 39.7	& 33.1	\\
painting	& 54.8	& 13.5	& -	& 50.3	& 50.4	& 41.5	\\
quickdraw	& 52.4	& 7.3	& 24.9	& -	& 41.8	& 35.3	\\
real    	& 59.5	& 16.4	& 42.4	& 52.5	& -	& 44.5	\\
sketch  	& 59.5	& 13.9	& 36.2	& 51.7	& 48.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.8	& 42.0	& 58.9	& 56.5	& 50.2	\\
infograph	& 57.2	& -	& 35.4	& 56.0	& 49.9	& 42.6	\\
painting	& 60.9	& 16.0	& -	& 57.2	& 56.2	& 48.0	\\
quickdraw	& 58.9	& 11.8	& 36.8	& -	& 52.0	& 44.2	\\
real    	& 64.9	& 18.8	& 47.2	& 58.6	& -	& 50.1	\\
sketch  	& 63.6	& 17.0	& 42.9	& 58.3	& 55.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 6.0	& 12.3	& 15.0	& 23.4	& 21.0	\\
infograph	& 10.2	& -	& 7.2	& 7.0	& 11.2	& 7.1	\\
painting	& 22.8	& 6.3	& -	& 8.3	& 28.7	& 17.1	\\
quickdraw	& 9.5	& 1.1	& 2.1	& -	& 5.1	& 4.9	\\
real    	& 35.4	& 9.2	& 26.4	& 9.8	& -	& 19.5	\\
sketch  	& 31.9	& 6.5	& 15.2	& 13.5	& 21.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 6.5	& 14.7	& 28.7	& 28.4	& 25.6	\\
infograph	& 17.4	& -	& 8.5	& 19.9	& 16.1	& 11.9	\\
painting	& 28.5	& 7.2	& -	& 23.1	& 31.8	& 22.3	\\
quickdraw	& 20.1	& 2.2	& 5.1	& -	& 12.5	& 12.1	\\
real    	& 39.7	& 9.9	& 27.1	& 24.1	& -	& 24.8	\\
sketch  	& 37.4	& 7.0	& 17.5	& 27.2	& 26.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 8.2	& 18.6	& 36.5	& 33.5	& 31.3	\\
infograph	& 24.2	& -	& 11.7	& 29.4	& 22.6	& 17.4	\\
painting	& 34.2	& 8.0	& -	& 32.7	& ??	& 27.9	\\
quickdraw	& 27.8	& 3.4	& 8.9	& -	& 20.5	& 18.6	\\
real    	& 43.4	& 11.1	& 29.6	& 33.7	& -	& 30.4	\\
sketch  	& 42.9	& 8.5	& 20.6	& 35.7	& 32.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.4	& 27.0	& 46.8	& 42.6	& 39.4	\\
infograph	& 37.1	& -	& 19.7	& 41.8	& 33.8	& 29.4	\\
painting	& 44.9	& 10.5	& -	& 44.2	& 43.3	& 36.8	\\
quickdraw	& 41.1	& 6.3	& 18.1	& -	& 32.4	& 29.7	\\
real    	& 49.8	& 13.4	& 34.0	& 45.2	& -	& 38.7	\\
sketch  	& 49.7	& 11.6	& 29.2	& 46.0	& 41.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.5	& 23.5	& 22.5	& 35.8	& 36.6	\\
infograph	& 23.9	& -	& 16.2	& 6.7	& 22.9	& 19.1	\\
painting	& 37.5	& 10.8	& -	& 8.8	& 41.8	& 29.8	\\
quickdraw	& 23.3	& 1.5	& 2.6	& -	& 9.5	& 10.9	\\
real    	& 45.2	& 12.3	& 36.3	& 12.6	& -	& 32.0	\\
sketch  	& 51.4	& 11.5	& 28.5	& 23.3	& 36.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 26.8	& 33.5	& 40.0	& 39.8	\\
infograph	& 33.3	& -	& 20.0	& 19.6	& 30.3	& 24.8	\\
painting	& 44.5	& 11.7	& -	& 21.6	& 45.8	& 34.0	\\
quickdraw	& 31.9	& 3.1	& 5.6	& -	& 16.5	& 18.9	\\
real    	& 50.8	& 13.4	& 39.1	& 30.7	& -	& 37.2	\\
sketch  	& 54.6	& 12.2	& 31.1	& 33.5	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.9	& 29.6	& 42.6	& 43.8	& 43.0	\\
infograph	& 40.6	& -	& 25.4	& 33.3	& 36.1	& 30.6	\\
painting	& 49.2	& 13.3	& -	& 32.4	& 48.9	& 38.6	\\
quickdraw	& 38.8	& 5.1	& 13.3	& -	& 22.3	& 24.8	\\
real    	& 55.3	& 15.2	& 40.7	& 39.4	& -	& 40.8	\\
sketch  	& 57.9	& 14.0	& 34.6	& 40.8	& 45.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.1	& 37.1	& 52.3	& 50.3	& 48.2	\\
infograph	& 51.4	& -	& 33.9	& 48.0	& 45.8	& 39.4	\\
painting	& 56.7	& 16.0	& -	& 46.7	& 54.6	& 44.8	\\
quickdraw	& 48.7	& 9.4	& 21.6	& -	& 38.0	& 37.4	\\
real    	& 60.2	& 17.9	& 45.4	& 51.0	& -	& 47.1	\\
sketch  	& 61.8	& 17.3	& 41.6	& 51.6	& 51.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.7	& 35.0	& 34.5	& 47.3	& 47.0	\\
infograph	& 37.9	& -	& 26.9	& 22.8	& 37.8	& 29.9	\\
painting	& 48.9	& 15.5	& -	& 28.5	& 51.0	& 43.3	\\
quickdraw	& 37.0	& 2.9	& 13.8	& -	& 27.8	& 24.1	\\
real    	& 59.6	& 17.9	& 47.9	& 36.5	& -	& 45.3	\\
sketch  	& 61.5	& 16.4	& 42.2	& 39.0	& 50.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 15.6	& 38.6	& 50.9	& 53.0	& 50.1	\\
infograph	& 48.1	& -	& 32.9	& 43.1	& 46.2	& 39.3	\\
painting	& 55.0	& 16.6	& -	& 44.8	& 56.0	& 48.3	\\
quickdraw	& 51.3	& 6.8	& 26.5	& -	& 43.0	& 36.4	\\
real    	& 65.0	& 19.4	& 49.8	& 51.7	& -	& 50.4	\\
sketch  	& 64.2	& 17.4	& 44.5	& 49.9	& 54.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 17.6	& 41.9	& 55.6	& 57.5	& 53.8	\\
infograph	& 53.2	& -	& 37.2	& 50.3	& 52.5	& 45.2	\\
painting	& 59.4	& 17.8	& -	& 52.6	& 59.9	& 51.2	\\
quickdraw	& 56.7	& 10.0	& 34.6	& -	& 51.0	& 44.5	\\
real    	& 67.6	& 20.9	& 51.8	& 56.9	& -	& 54.3	\\
sketch  	& 66.4	& 19.4	& 47.2	& 55.8	& 58.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 20.8	& 49.2	& 62.0	& 64.2	& 58.1	\\
infograph	& 61.5	& -	& 44.9	& 58.4	& 60.9	& 51.5	\\
painting	& 65.3	& 21.0	& -	& 59.5	& 66.2	& 56.9	\\
quickdraw	& 64.1	& 14.8	& 44.5	& -	& 61.1	& 52.6	\\
real    	& 71.1	& 24.2	& 56.1	& 62.9	& -	& 58.6	\\
sketch  	& 70.6	& 22.7	& 52.4	& 61.9	& 64.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 25.2	& 22.5	& 36.4	& 38.2	\\
infograph	& 24.9	& -	& 17.1	& 14.3	& 24.3	& 20.9	\\
painting	& 39.7	& 12.2	& -	& 17.7	& 44.2	& 34.1	\\
quickdraw	& 24.7	& 2.4	& 7.4	& -	& 15.2	& 15.8	\\
real    	& 47.9	& 14.7	& 40.4	& 20.2	& -	& 35.1	\\
sketch  	& 51.4	& 12.1	& 31.4	& 20.5	& 37.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.8	& 29.8	& 39.8	& 42.9	& 43.2	\\
infograph	& 38.9	& -	& 22.2	& 33.7	& 34.5	& 29.9	\\
painting	& 49.4	& 13.7	& -	& 36.0	& 50.2	& 40.4	\\
quickdraw	& 38.6	& 5.2	& 15.8	& -	& 27.4	& 25.9	\\
real    	& 56.0	& 15.8	& 43.0	& 37.9	& -	& 41.6	\\
sketch  	& 57.6	& 13.8	& 34.7	& 38.5	& 43.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.5	& 33.9	& 47.5	& 48.6	& 47.5	\\
infograph	& 47.3	& -	& 27.1	& 43.6	& 41.8	& 36.7	\\
painting	& 55.0	& 15.5	& -	& 45.1	& 54.2	& 45.2	\\
quickdraw	& 46.1	& 7.8	& 21.9	& -	& 37.1	& 33.9	\\
real    	& 59.9	& 18.0	& 45.7	& 46.3	& -	& 46.9	\\
sketch  	& 61.0	& 15.7	& 38.3	& 47.3	& 49.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 18.1	& 43.0	& 56.5	& 57.0	& 53.8	\\
infograph	& 59.5	& -	& 38.3	& 54.0	& 53.8	& 47.7	\\
painting	& 63.5	& 18.9	& -	& 55.3	& 60.9	& 52.5	\\
quickdraw	& 57.3	& 12.9	& 35.2	& -	& 49.6	& 44.8	\\
real    	& 66.3	& 21.3	& 51.2	& 56.0	& -	& 53.9	\\
sketch  	& 67.0	& 20.4	& 46.2	& 56.0	& 57.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.5	& 28.6	& 30.2	& 41.3	& 41.6	\\
infograph	& 27.8	& -	& 17.4	& 17.8	& 25.9	& 22.0	\\
painting	& 43.6	& 12.2	& -	& 23.3	& 45.9	& 35.1	\\
quickdraw	& 35.3	& 2.5	& 10.5	& -	& 19.7	& 18.3	\\
real    	& 51.2	& 14.4	& 40.9	& 25.9	& -	& 37.2	\\
sketch  	& 54.9	& 12.7	& 33.1	& 28.2	& 39.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.0	& 40.3	& 55.3	& 54.6	& 51.8	\\
infograph	& 55.1	& -	& 30.7	& 50.5	& 46.6	& 41.5	\\
painting	& 60.3	& 15.4	& -	& 52.6	& 56.4	& 48.6	\\
quickdraw	& 56.5	& 8.9	& 31.1	& -	& 46.1	& 41.4	\\
real    	& 64.2	& 18.0	& 47.0	& 53.3	& -	& 49.6	\\
sketch  	& 64.8	& 16.0	& 42.7	& 54.3	& 54.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 5.5	& 11.2	& 16.0	& 22.0	& 18.8	\\
infograph	& 9.1	& -	& 6.1	& 7.2	& 9.7	& 4.6	\\
painting	& 20.8	& 5.5	& -	& 9.6	& 27.4	& 13.8	\\
quickdraw	& 8.4	& 1.0	& 1.5	& -	& 3.8	& 4.3	\\
real    	& 35.8	& 9.4	& 27.2	& 12.6	& -	& 19.8	\\
sketch  	& 32.5	& 6.2	& 15.2	& 17.6	& 22.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 5.8	& 12.4	& 29.2	& 24.6	& 23.0	\\
infograph	& 13.9	& -	& 7.1	& 22.5	& 13.5	& 7.1	\\
painting	& 23.7	& 5.8	& -	& 25.7	& 29.0	& 15.3	\\
quickdraw	& 16.9	& 1.9	& 3.0	& -	& 9.9	& 9.6	\\
real    	& 38.6	& 9.7	& 26.5	& 26.4	& -	& 22.3	\\
sketch  	& 36.3	& 6.1	& 15.6	& 29.0	& 25.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.0	& 14.3	& 37.8	& 30.5	& 28.2	\\
infograph	& 20.8	& -	& 9.2	& 32.0	& 19.2	& 15.5	\\
painting	& 29.3	& 6.8	& -	& 33.2	& 33.3	& 24.1	\\
quickdraw	& 26.0	& 2.9	& 5.8	& -	& 16.8	& 17.6	\\
real    	& 42.9	& 10.8	& 28.9	& 34.5	& -	& 27.8	\\
sketch  	& 42.5	& 7.0	& 17.5	& 38.4	& 31.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.3	& 22.6	& 46.7	& 41.2	& 39.5	\\
infograph	& 34.2	& -	& 16.9	& 43.5	& 30.8	& 29.9	\\
painting	& 42.6	& 8.9	& -	& 45.7	& 42.7	& 37.9	\\
quickdraw	& 40.4	& 5.3	& 15.4	& -	& 30.5	& 30.6	\\
real    	& 50.1	& 12.9	& 34.3	& 46.2	& -	& 38.4	\\
sketch  	& 50.6	& 11.2	& 28.0	& 47.0	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.1	& 28.8	& 24.9	& 39.8	& 42.6	\\
infograph	& 27.5	& -	& 19.9	& 8.1	& 25.5	& 22.1	\\
painting	& 40.9	& 11.0	& -	& 9.7	& 43.9	& 33.5	\\
quickdraw	& 25.8	& 2.0	& 6.1	& -	& 12.7	& 15.9	\\
real    	& 48.1	& 13.1	& 41.1	& 14.4	& -	& 34.0	\\
sketch  	& 56.5	& 13.7	& 37.1	& 27.0	& 43.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.3	& 31.9	& 36.4	& 44.3	& 45.8	\\
infograph	& 39.7	& -	& 25.4	& 26.5	& 36.0	& 29.9	\\
painting	& 48.7	& 12.9	& -	& 24.5	& 49.9	& 38.0	\\
quickdraw	& 35.1	& 4.3	& 15.0	& -	& 25.8	& 24.2	\\
real    	& 54.8	& 14.4	& 43.5	& 32.7	& -	& 40.6	\\
sketch  	& 59.2	& 14.4	& 39.4	& 37.5	& 46.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 18.8	& 43.0	& 53.0	& 55.3	& 53.7	\\
infograph	& 58.0	& -	& 39.4	& 51.6	& 50.8	& 46.4	\\
painting	& 61.5	& 17.9	& -	& 49.9	& 57.3	& 49.6	\\
quickdraw	& 54.5	& 11.8	& 33.7	& -	& 47.2	& 42.6	\\
real    	& 64.0	& 20.0	& 49.6	& 54.0	& -	& 51.6	\\
sketch  	& 65.9	& 20.3	& 48.4	& 53.8	& 55.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

% data/NextMatch Results - SSDA.csv
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive	& DigitFive	& DigitFive	& DigitFive	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet224	& DomainNet224	& DomainNet224	& DomainNet224	\\
& 25	& 10	& 1	& 5	& 10	& 5	& 25	& 1	& 25	& 5	& 1	& 10	\\
\\
\midrule
BaselineBN	& 89.4	& 85.7	& 73.4	& 81.0	& 34.0	& 28.6	& 42.1	& 20.8	& 47.6	& 33.8	& 25.3	& 39.3	\\
MCD     	& nan	& nan	& nan	& nan	& 24.3	& 19.5	& 33.2	& 13.8	& 32.5	& 17.8	& 13.5	& 23.1	\\
NoisyStudent	& 80.5	& 76.4	& 72.8	& 75.3	& 33.6	& 28.6	& 41.4	& 22.8	& 46.0	& 33.0	& 26.0	& nan	\\
FixMatch+	& 97.9	& 98.1	& 83.1	& 97.8	& 39.6	& 34.2	& 46.1	& 24.8	& nan	& nan	& 28.3	& 44.1	\\
AdaMatch	& 97.7	& 98.0	& 97.9	& 98.0	& 40.6	& 36.5	& 46.4	& 30.4	& 52.8	& 42.3	& 34.8	& 46.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}



%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 10.1	\\
svhn    	& 39.8	\\
syndigit	& 99.2	\\
usps    	& 96.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 98.0	\\
mnistm  	& 97.3	\\
svhn    	& 96.3	\\
syndigit	& 99.1	\\
usps    	& 95.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 97.1	\\
svhn    	& 95.7	\\
syndigit	& 99.4	\\
usps    	& 96.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.2	\\
syndigit	& 97.8	\\
usps    	& 97.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 64.4	\\
mnistm  	& 14.6	\\
svhn    	& 16.9	\\
syndigit	& 41.0	\\
usps    	& 63.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 83.2	\\
mnistm  	& 29.9	\\
svhn    	& 36.5	\\
syndigit	& 77.9	\\
usps    	& 81.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 91.1	\\
mnistm  	& 51.5	\\
svhn    	& 54.0	\\
syndigit	& 83.5	\\
usps    	& 88.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 95.3	\\
mnistm  	& 78.3	\\
svhn    	& 69.5	\\
syndigit	& 94.4	\\
usps    	& 94.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 9.9	\\
svhn    	& 31.5	\\
syndigit	& 37.9	\\
usps    	& 80.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 97.4	\\
svhn    	& 82.2	\\
syndigit	& 99.1	\\
usps    	& 97.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.3	\\
mnistm  	& 98.9	\\
svhn    	& 96.8	\\
syndigit	& 99.5	\\
usps    	& 97.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.9	\\
syndigit	& 99.4	\\
usps    	& 97.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 61.6	\\
mnistm  	& 10.4	\\
svhn    	& 8.5	\\
syndigit	& 9.7	\\
usps    	& 46.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 90.9	\\
mnistm  	& 18.8	\\
svhn    	& 11.5	\\
syndigit	& 40.5	\\
usps    	& 92.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 94.8	\\
mnistm  	& 80.4	\\
svhn    	& 31.4	\\
syndigit	& 92.4	\\
usps    	& 92.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.1	\\
mnistm  	& 94.4	\\
svhn    	& 82.3	\\
syndigit	& 96.6	\\
usps    	& 94.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 71.2	\\
mnistm  	& 13.1	\\
svhn    	& 16.2	\\
syndigit	& 40.8	\\
usps    	& 75.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 91.0	\\
mnistm  	& 29.6	\\
svhn    	& 41.9	\\
syndigit	& 84.5	\\
usps    	& 89.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 96.8	\\
mnistm  	& 59.9	\\
svhn    	& 62.0	\\
syndigit	& 90.9	\\
usps    	& 92.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 90.5	\\
svhn    	& 80.0	\\
syndigit	& 95.9	\\
usps    	& 96.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.5	\\
infograph	& 1.5	\\
painting	& 3.9	\\
quickdraw	& 18.7	\\
real    	& 8.3	\\
sketch  	& 6.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 41.5	\\
infograph	& 4.0	\\
painting	& 13.0	\\
quickdraw	& 42.0	\\
real    	& 28.6	\\
sketch  	& 25.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 51.8	\\
infograph	& 5.8	\\
painting	& 21.7	\\
quickdraw	& 51.5	\\
real    	& 42.4	\\
sketch  	& 36.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 62.6	\\
infograph	& 10.3	\\
painting	& 39.5	\\
quickdraw	& 59.8	\\
real    	& 56.5	\\
sketch  	& 49.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 7.4	\\
infograph	& 1.3	\\
painting	& 3.4	\\
quickdraw	& 14.5	\\
real    	& 7.0	\\
sketch  	& 5.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 26.6	\\
infograph	& 3.3	\\
painting	& 9.1	\\
quickdraw	& 33.1	\\
real    	& 20.1	\\
sketch  	& 16.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 37.9	\\
infograph	& 5.0	\\
painting	& 13.5	\\
quickdraw	& 42.6	\\
real    	& 31.1	\\
sketch  	& 26.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 53.2	\\
infograph	& 8.2	\\
painting	& 28.0	\\
quickdraw	& 53.8	\\
real    	& 46.2	\\
sketch  	& 41.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 2.3	\\
infograph	& 0.9	\\
painting	& 1.7	\\
quickdraw	& 7.5	\\
real    	& 3.0	\\
sketch  	& 1.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 9.2	\\
infograph	& 1.9	\\
painting	& 3.8	\\
quickdraw	& 25.1	\\
real    	& 9.3	\\
sketch  	& 4.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 16.4	\\
infograph	& 3.4	\\
painting	& 7.1	\\
quickdraw	& 35.7	\\
real    	& 16.2	\\
sketch  	& 10.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 31.8	\\
infograph	& 5.7	\\
painting	& 15.1	\\
quickdraw	& 47.4	\\
real    	& 28.8	\\
sketch  	& 27.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 36.4	\\
infograph	& 3.9	\\
painting	& 13.6	\\
quickdraw	& 39.8	\\
real    	& 27.8	\\
sketch  	& 24.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.3	\\
infograph	& 5.6	\\
painting	& 20.9	\\
quickdraw	& 49.6	\\
real    	& 41.5	\\
sketch  	& 35.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 60.8	\\
infograph	& 9.7	\\
painting	& 38.8	\\
quickdraw	& 59.4	\\
real    	& 55.2	\\
sketch  	& 48.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.2	\\
infograph	& 1.5	\\
painting	& 4.0	\\
quickdraw	& 18.9	\\
real    	& 8.5	\\
sketch  	& 5.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 36.5	\\
infograph	& 3.6	\\
painting	& 13.3	\\
quickdraw	& 41.7	\\
real    	& 26.9	\\
sketch  	& 21.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 46.4	\\
infograph	& 5.8	\\
painting	& 20.8	\\
quickdraw	& 49.9	\\
real    	& 37.9	\\
sketch  	& 29.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 56.2	\\
infograph	& 9.3	\\
painting	& 33.3	\\
quickdraw	& 57.7	\\
real    	& 50.3	\\
sketch  	& 41.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 6.9	\\
infograph	& 1.4	\\
painting	& 3.1	\\
quickdraw	& 13.2	\\
real    	& 6.6	\\
sketch  	& 4.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 23.6	\\
infograph	& 3.2	\\
painting	& 9.1	\\
quickdraw	& 31.2	\\
real    	& 18.2	\\
sketch  	& 13.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 33.9	\\
infograph	& 4.8	\\
painting	& 14.2	\\
quickdraw	& 40.3	\\
real    	& 28.2	\\
sketch  	& 22.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.2	\\
infograph	& 7.8	\\
painting	& 25.7	\\
quickdraw	& 51.1	\\
real    	& 41.5	\\
sketch  	& 34.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 9.7	\\
infograph	& 1.4	\\
painting	& 3.9	\\
quickdraw	& 17.1	\\
real    	& 7.5	\\
sketch  	& 6.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 37.6	\\
infograph	& 3.5	\\
painting	& 13.1	\\
quickdraw	& 42.3	\\
real    	& 27.2	\\
sketch  	& 21.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.1	\\
infograph	& 5.3	\\
painting	& 18.9	\\
quickdraw	& 50.9	\\
real    	& 39.0	\\
sketch  	& 30.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 57.2	\\
infograph	& 8.8	\\
painting	& 32.7	\\
quickdraw	& 58.0	\\
real    	& 50.5	\\
sketch  	& 41.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 3.0	\\
infograph	& 1.0	\\
painting	& 1.8	\\
quickdraw	& 7.8	\\
real    	& 3.5	\\
sketch  	& 1.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.5	\\
infograph	& 2.3	\\
painting	& 5.0	\\
quickdraw	& 25.1	\\
real    	& 11.3	\\
sketch  	& 6.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 19.6	\\
infograph	& 3.5	\\
painting	& 9.5	\\
quickdraw	& 35.1	\\
real    	& 18.7	\\
sketch  	& 13.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 34.7	\\
infograph	& 5.6	\\
painting	& 17.3	\\
quickdraw	& 47.1	\\
real    	& 32.3	\\
sketch  	& 27.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 8.7	\\
infograph	& 1.5	\\
painting	& 4.1	\\
quickdraw	& 16.7	\\
real    	& 7.6	\\
sketch  	& 5.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 31.8	\\
infograph	& 3.5	\\
painting	& 11.8	\\
quickdraw	& 37.1	\\
real    	& 24.3	\\
sketch  	& 17.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 42.3	\\
infograph	& 5.3	\\
painting	& 18.6	\\
quickdraw	& 46.7	\\
real    	& 35.6	\\
sketch  	& 27.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 54.6	\\
infograph	& 8.7	\\
painting	& 31.7	\\
quickdraw	& 57.4	\\
real    	& 49.4	\\
sketch  	& 40.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

% ['data/NextMatch Results - SSL.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive	& DigitFive	& DigitFive	& DigitFive	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet224	& DomainNet224	& DomainNet224	& DomainNet224	\\
& 10	& 5	& 25	& 1	& 25	& 5	& 1	& 10	& 10	& 5	& 25	& 1	\\
\\
\midrule
BaselineBN	& 73.7	& 61.9	& 86.4	& 40.0	& 34.9	& 16.5	& 5.9	& 23.9	& 26.2	& 18.1	& 38.5	& 6.5	\\
MCD     	& 78.4	& 50.8	& 93.0	& 27.4	& 27.5	& 10.2	& 3.1	& 16.7	& 14.9	& 8.9	& 26.0	& 2.8	\\
NoisyStudent	& 80.5	& 67.4	& 92.1	& 43.3	& 40.3	& 21.1	& 7.3	& 29.3	& 33.6	& 24.2	& 45.4	& nan	\\
FixMatch+	& 98.3	& 94.8	& 98.1	& 51.5	& 41.5	& 24.1	& 7.6	& 32.1	& nan	& nan	& nan	& nan	\\
AdaMatch	& 97.6	& 97.2	& 97.6	& 68.6	& 41.4	& 23.8	& 8.1	& 31.7	& 34.9	& 25.7	& 46.4	& 8.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.8	& 35.3	& 26.8	& 46.5	& 46.5	\\
infograph	& 21.7	& -	& 11.7	& 0.3	& 20.0	& 0.2	\\
painting	& 45.3	& 13.5	& -	& 13.2	& 48.1	& 41.0	\\
quickdraw	& 33.6	& 2.4	& 10.1	& -	& 19.1	& 21.1	\\
real    	& 56.0	& 16.6	& 47.6	& 22.9	& -	& 42.4	\\
sketch  	& 60.2	& 17.0	& 42.9	& 34.2	& 49.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.4	& 23.4	& 12.1	& 33.4	& 34.9	\\
infograph	& 16.2	& -	& 13.8	& 0.9	& 16.5	& 11.5	\\
painting	& 33.6	& 11.2	& -	& 1.0	& 41.2	& 25.7	\\
quickdraw	& 11.2	& 0.8	& 2.5	& -	& 5.5	& 7.1	\\
real    	& 43.4	& 13.7	& 39.4	& 2.1	& -	& 29.6	\\
sketch  	& 47.9	& 11.0	& 28.7	& 3.8	& 33.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.6	& 26.4	& 11.2	& 37.6	& 37.8	\\
infograph	& 15.8	& -	& 6.5	& 0.6	& 8.6	& 11.4	\\
painting	& 39.0	& 11.6	& -	& 4.2	& 42.7	& 31.4	\\
quickdraw	& 15.8	& 1.3	& 5.0	& -	& 11.5	& 12.2	\\
real    	& 48.1	& 13.8	& 39.8	& 7.3	& -	& 33.4	\\
sketch  	& 50.3	& 11.8	& 30.7	& 11.8	& 34.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.7	& 15.2	& 15.2	& 25.8	& 23.4	\\
infograph	& 9.2	& -	& 7.0	& 1.6	& 11.2	& 6.5	\\
painting	& 25.6	& 7.0	& -	& 5.3	& 32.1	& 18.8	\\
quickdraw	& 7.4	& 0.7	& 0.7	& -	& 1.6	& 4.1	\\
real    	& 38.4	& 10.5	& 32.4	& 7.7	& -	& 22.9	\\
sketch  	& 37.2	& 8.2	& 22.9	& 14.7	& 26.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.9	& 28.5	& 20.4	& 39.5	& 42.3	\\
infograph	& 24.5	& -	& 18.9	& 3.1	& 23.9	& 18.3	\\
painting	& 37.6	& 11.4	& -	& 3.4	& 40.9	& 30.9	\\
quickdraw	& 20.9	& 1.0	& 2.7	& -	& 8.7	& 13.2	\\
real    	& 47.8	& 13.7	& 39.8	& 7.7	& -	& 32.6	\\
sketch  	& 55.2	& 14.8	& 37.1	& 22.8	& 41.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_None }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.2	& 29.3	& 27.9	& 40.8	& 40.6	\\
infograph	& 22.1	& -	& 18.5	& 6.2	& 24.2	& 19.8	\\
painting	& 39.6	& 11.7	& -	& 12.6	& 43.4	& 34.9	\\
quickdraw	& 24.6	& 2.4	& 8.4	& -	& 16.4	& 15.5	\\
real    	& 52.2	& 15.0	& 41.6	& 13.3	& -	& 38.6	\\
sketch  	& 53.4	& 13.6	& 35.6	& 25.4	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.5	& 19.0	& 6.3	& 29.4	& 29.9	\\
infograph	& 12.9	& -	& 10.8	& 0.6	& 14.0	& 9.5	\\
painting	& 27.3	& 9.3	& -	& 1.0	& 36.3	& 21.8	\\
quickdraw	& 10.3	& 0.8	& 1.9	& -	& 4.8	& 5.9	\\
real    	& 39.3	& 11.9	& 34.6	& 2.2	& -	& 25.5	\\
sketch  	& 40.9	& 8.5	& 20.4	& 3.3	& 26.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.2	& 24.6	& 14.6	& 35.7	& 35.3	\\
infograph	& 17.9	& -	& 14.3	& 2.2	& 18.7	& 14.2	\\
painting	& 34.7	& 10.7	& -	& 4.2	& 39.7	& 27.7	\\
quickdraw	& 23.7	& 1.4	& 5.1	& -	& 11.2	& 10.2	\\
real    	& 45.4	& 13.5	& 37.4	& 6.6	& -	& 30.7	\\
sketch  	& 48.1	& 10.3	& 26.6	& 10.4	& 31.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.5	& 15.9	& 12.9	& 26.2	& 25.6	\\
infograph	& 11.3	& -	& 9.4	& 2.3	& 13.3	& 8.6	\\
painting	& 25.8	& 7.5	& -	& 4.3	& 32.1	& 21.4	\\
quickdraw	& 8.0	& 0.6	& 0.6	& -	& 1.6	& 4.6	\\
real    	& 37.2	& 10.1	& 29.8	& 6.8	& -	& 22.9	\\
sketch  	& 37.3	& 7.8	& 20.2	& 11.6	& 25.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.9	& 24.3	& 18.9	& 35.4	& 36.8	\\
infograph	& 21.2	& -	& 16.9	& 2.6	& 21.8	& 16.0	\\
painting	& 36.1	& 11.7	& -	& 3.6	& 41.5	& 28.5	\\
quickdraw	& 19.0	& 0.9	& 1.5	& -	& 6.8	& 7.2	\\
real    	& 44.0	& 13.8	& 38.3	& 6.6	& -	& 30.6	\\
sketch  	& 50.0	& 12.0	& 30.4	& 18.2	& 36.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_None }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.6	& 97.6	\\
mnistm  	& 96.7	\\
svhn    	& 99.3	\\
syndigit	& 96.9	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 54.3	& 55.0	& 76.0	& 96.3	\\
mnistm  	& 96.5	& -	& 52.4	& 81.8	& 88.1	\\
svhn    	& 40.4	& 32.0	& -	& 86.3	& 39.9	\\
syndigit	& 67.7	& 30.0	& 79.7	& -	& 70.5	\\
usps    	& 78.6	& 27.3	& 31.9	& 64.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 97.0	& 97.9	\\
mnistm  	& 96.8	\\
svhn    	& 99.2	\\
syndigit	& 96.9	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 13.1	& 9.7	& 91.2	\\
mnistm  	& 16.9	\\
svhn    	& 81.3	\\
syndigit	& 84.3	\\
usps    	& 94.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 30.4	& 51.4	& 81.8	& 97.2	\\
mnistm  	& 99.2	& -	& 63.0	& 89.0	& 97.0	\\
svhn    	& 82.8	& 45.2	& -	& 98.9	& 83.9	\\
syndigit	& 92.6	& 50.5	& 90.0	& -	& 87.1	\\
usps    	& 95.5	& 25.2	& 30.0	& 75.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_None }
\end{table}

% ['data/NextMatch Results - DA - DigitFive (MCD).csv', 'data/NextMatch Results - DA.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrr}
\toprule
& DigitFive	& DomainNet64	& DomainNet224	\\
& 1	& 1	& 1	\\
\\
\midrule
BaselineBN	& 62.5	& 15.8	& 18.9	\\
MCD     	& 55.9	& 14.9	& 14.9	\\
NoisyStudent	& 73.3	& 21.4	& 23.9	\\
FixMatch+	& 98.1	& 20.6	& 20.8	\\
AdaMatch	& 97.9	& 26.0	& 28.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}

%% run {'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FSL}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.3	& 19.3	& 15.0	& 30.1	& 31.9	\\
infograph	& 14.7	& -	& 11.2	& 2.1	& 15.3	& 11.4	\\
painting	& 29.8	& 9.1	& -	& 2.8	& 37.6	& 24.0	\\
quickdraw	& 14.5	& 0.8	& 0.9	& -	& 4.9	& 5.9	\\
real    	& 42.5	& 13.2	& 36.9	& 6.5	& -	& 27.9	\\
sketch  	& 43.0	& 9.2	& 22.4	& 13.6	& 28.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FSL }
\end{table}

%% run {'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FSL}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.6	& 24.6	& 16.4	& 35.6	& 38.1	\\
infograph	& 21.3	& -	& 16.3	& 3.4	& 21.8	& 17.1	\\
painting	& 37.6	& 11.5	& -	& 5.4	& 44.4	& 31.4	\\
quickdraw	& 15.3	& 0.8	& 1.7	& -	& 5.4	& 8.7	\\
real    	& 48.0	& 15.8	& 44.1	& 8.0	& -	& 34.5	\\
sketch  	& 50.0	& 11.7	& 31.7	& 17.1	& 36.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FSL }
\end{table}

%% run {'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Oracle}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 31.6	& 60.0	& 70.7	& 70.7	& 62.5	\\
infograph	& 70.0	& -	& 58.2	& 69.8	& 69.2	& 60.1	\\
painting	& 71.9	& 32.3	& -	& 70.3	& 71.0	& 62.3	\\
quickdraw	& 70.2	& 29.5	& 58.3	& -	& 69.1	& 60.3	\\
real    	& 73.5	& 33.8	& 61.9	& nan	& -	& 63.3	\\
sketch  	& 72.3	& 31.9	& 60.2	& 70.6	& 70.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Oracle }
\end{table}

%% run {'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Oracle}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 38.8	& 65.9	& 71.9	& 74.8	& 69.0	\\
infograph	& 75.8	& -	& 65.7	& 71.4	& 74.5	& 67.7	\\
painting	& 76.9	& 39.1	& -	& 71.8	& 75.6	& 68.4	\\
quickdraw	& 74.5	& 35.7	& 63.4	& -	& 72.7	& 66.2	\\
real    	& 77.8	& 40.6	& 67.7	& 71.9	& -	& 69.2	\\
sketch  	& 77.3	& 39.5	& 66.1	& 72.1	& 74.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Oracle }
\end{table}

%% run {'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FSL}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 23.3	& 33.9	& 72.9	& 95.9	\\
mnistm  	& 98.7	& -	& 43.9	& 83.0	& 96.2	\\
svhn    	& 72.1	& 37.3	& -	& 98.2	& 75.2	\\
syndigit	& 88.5	& 30.6	& 80.1	& -	& 78.0	\\
usps    	& 81.8	& 15.0	& 23.3	& 69.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FSL }
\end{table}

%% run {'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Oracle}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 99.2	& 97.5	& 99.9	& 98.1	\\
mnistm  	& 99.5	& -	& 97.6	& 99.9	& 98.0	\\
svhn    	& 99.4	& 99.1	& -	& 99.9	& 97.6	\\
syndigit	& 99.5	& 99.1	& 97.6	& -	& 97.6	\\
usps    	& 99.5	& 99.2	& 97.5	& 99.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Oracle }
\end{table}


==> autogenerated_figures.tex <==
% ['data/NextMatch Results - DA.csv', 'data/NextMatch Results - DA - DigitFive.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrr}
\toprule
& DigitFive     & DomainNet64   & DomainNet224  \\
& 1     & 1     & 1     \\
\\
\midrule
BaselineBN      & nan   & 15.8  & 18.9  \\
MCD             & 57.8  & 14.9  & 14.9  \\
NoisyStudent    & 73.3  & 21.0  & 23.6  \\
FixMatch+       & 92.9  & 21.6  & 21.3  \\
AdaMatch        & 97.8  & 26.0  & 28.7  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


% ['data/NextMatch Results - SSL.csv', 'data/NextMatch Results - SSL - DigitFive.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive     & DigitFive     & DigitFive     & DigitFive     & DomainNet64   & DomainNet64   & DomainNet64   & DomainNet64   & DomainNet224  & DomainNet224  & DomainNet224  & DomainNet224  \\
& 1     & 25    & 5     & 10    & 10    & 5     & 1     & 25    & 10    & 5     & 1     & 25    \\
\\
\midrule
BaselineBN      & nan   & nan   & nan   & nan   & 23.9  & 16.5  & 5.9   & 34.9  & 26.2  & 18.1  & 6.5   & 38.5  \\
MCD             & 27.4  & 93.0  & 50.8  & 78.4  & 16.7  & 10.2  & 3.1   & 27.5  & 14.9  & 8.9   & 2.8   & 26.0  \\
NoisyStudent    & 43.3  & 92.1  & 67.4  & 80.5  & 29.3  & 21.1  & 7.3   & 40.3  & nan   & nan   & nan   & nan   \\
FixMatch+       & 60.8  & 98.2  & 95.0  & 98.3  & 32.3  & 24.1  & 7.7   & 41.3  & 32.8  & 23.8  & 7.6   & 43.0  \\
AdaMatch        & 68.6  & 97.6  & 97.2  & 97.6  & 31.7  & 23.8  & 8.1   & 41.4  & 34.9  & 25.7  & 8.2   & 46.4  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


% data/NextMatch Results - SSDA.csv
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
& \multicolumn{4}{c}{DomainNet64}  & \multicolumn{4}{c}{DomainNet224} \\
& 5     & 25    & 10    & 1     & 25    & 5     & 1     & 10    \\
\\
\midrule
BaselineBN      & 28.6  & 42.1  & 34.0  & 20.8  & 47.6  & 33.8  & 25.3  & 39.3  \\
MCD             & 19.5  & 33.2  & 24.3  & 13.8  & 32.5  & 17.8  & 13.5  & 23.1  \\
NoisyStudent    & 28.6  & 41.4  & 33.6  & 22.8  & nan   & nan   & nan   & nan   \\
FixMatch+       & 37.0  & 47.4  & 41.8  & 28.2  & 51.0  & 41.5  & 31.0  & 46.7  \\
AdaMatch        & 36.5  & 46.4  & 40.6  & 30.4  & 52.8  & 42.3  & 34.8  & 46.7  \\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> new_autogenerated.tex <==
%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.8	& 97.7	\\
mnistm  	& 96.5	\\
svhn    	& 99.2	\\
syndigit	& 96.9	\\
usps    	& 99.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.1	& 96.6	& 97.8	\\
mnistm  	& 96.7	\\
svhn    	& 99.2	\\
syndigit	& 96.8	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.7	& 97.9	\\
mnistm  	& 96.7	\\
svhn    	& 99.3	\\
syndigit	& 96.7	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.1	& 96.1	& 97.7	\\
mnistm  	& 96.3	\\
svhn    	& 99.3	\\
syndigit	& 96.3	\\
usps    	& 99.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 72.4	& 42.0	& 95.8	\\
mnistm  	& 63.6	\\
svhn    	& 79.8	\\
syndigit	& 76.2	\\
usps    	& 83.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 81.0	& 59.3	& 96.2	\\
mnistm  	& 68.5	\\
svhn    	& 90.5	\\
syndigit	& 80.8	\\
usps    	& 90.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 86.3	& 68.2	& 96.5	\\
mnistm  	& 74.7	\\
svhn    	& 94.7	\\
syndigit	& 84.5	\\
usps    	& 95.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 92.7	& 77.4	& 97.0	\\
mnistm  	& 78.7	\\
svhn    	& 96.8	\\
syndigit	& 86.2	\\
usps    	& 96.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 58.6	& 97.9	\\
mnistm  	& 31.9	\\
svhn    	& 97.9	\\
syndigit	& 97.0	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.9	& 97.8	\\
mnistm  	& 96.9	\\
svhn    	& 97.9	\\
syndigit	& 96.8	\\
usps    	& 99.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.8	& 98.1	\\
mnistm  	& 96.9	\\
svhn    	& 99.3	\\
syndigit	& 97.0	\\
usps    	& 99.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.5	& 97.9	\\
mnistm  	& 96.5	\\
svhn    	& 99.2	\\
syndigit	& 96.6	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 32.8	& 59.7	& 71.8	& 94.0	\\
mnistm  	& 99.2	& -	& 58.6	& 88.0	& 95.1	\\
svhn    	& 80.2	& 44.2	& -	& 98.8	& 85.9	\\
syndigit	& 91.8	& 51.4	& 88.8	& -	& 88.1	\\
usps    	& 95.5	& 25.3	& 33.4	& 73.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 28.1	& 63.1	& 88.6	& 95.0	\\
mnistm  	& 99.2	& -	& 64.9	& 90.1	& 93.1	\\
svhn    	& 80.7	& 49.6	& -	& 98.9	& 85.3	\\
syndigit	& 92.5	& 62.3	& 89.3	& -	& 86.6	\\
usps    	& 94.2	& 30.4	& 38.2	& 76.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 26.8	& 59.9	& 86.8	& 96.9	\\
mnistm  	& 99.3	& -	& 62.8	& 88.5	& 95.7	\\
svhn    	& 78.5	& 58.0	& -	& 98.9	& 88.8	\\
syndigit	& 92.5	& 70.9	& 89.4	& -	& 87.9	\\
usps    	& 94.2	& 31.8	& 41.4	& 78.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 32.2	& 66.7	& 87.6	& 96.9	\\
mnistm  	& 99.2	& -	& 79.3	& 91.7	& 95.6	\\
svhn    	& 86.6	& 68.9	& -	& 98.8	& 89.2	\\
syndigit	& 93.4	& 75.3	& 90.5	& -	& 89.2	\\
usps    	& 94.9	& 62.7	& 34.0	& 78.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 28.1	& 37.1	& 40.7	& 39.7	\\
infograph	& 29.2	& -	& 20.5	& 23.3	& 31.0	& 24.1	\\
painting	& 42.8	& 12.6	& -	& 26.5	& 44.7	& 36.4	\\
quickdraw	& 35.7	& 2.6	& 13.2	& -	& 25.1	& 22.2	\\
real    	& 54.6	& 15.3	& 40.7	& 34.0	& -	& 39.2	\\
sketch  	& 54.7	& 13.6	& 34.9	& 35.7	& 43.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.4	& 30.4	& 47.8	& 45.8	& 42.1	\\
infograph	& 40.4	& -	& 24.1	& 39.4	& 38.5	& 29.7	\\
painting	& 48.5	& 12.9	& -	& 41.4	& 48.5	& 39.6	\\
quickdraw	& 46.8	& 5.4	& 21.2	& -	& 37.0	& 30.4	\\
real    	& 58.5	& 15.8	& 42.4	& 49.1	& -	& 43.3	\\
sketch  	& 58.1	& 13.5	& 36.9	& 46.6	& 47.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.9	& 34.4	& 52.9	& 49.7	& 45.3	\\
infograph	& 45.9	& -	& 28.3	& 47.6	& 43.3	& 35.8	\\
painting	& 52.8	& 14.3	& -	& 49.0	& 52.0	& 43.2	\\
quickdraw	& 52.0	& 7.2	& 27.3	& -	& 44.3	& 36.8	\\
real    	& 61.2	& 17.5	& 44.7	& 54.9	& -	& 46.5	\\
sketch  	& 60.1	& 15.1	& 39.4	& 52.8	& 50.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.8	& 40.7	& 59.0	& 56.5	& 50.3	\\
infograph	& 54.5	& -	& 35.1	& 55.4	& 51.7	& 42.7	\\
painting	& 58.6	& 16.3	& -	& 56.5	& 57.8	& 48.7	\\
quickdraw	& 58.1	& 12.0	& 37.0	& -	& 53.5	& 44.3	\\
real    	& 65.5	& 19.5	& 47.9	& 60.7	& -	& 51.2	\\
sketch  	& 64.0	& 17.6	& 43.8	& 58.9	& 56.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.3	& 19.7	& 22.2	& 31.1	& 31.1	\\
infograph	& 18.1	& -	& 11.8	& 11.4	& 17.4	& 14.1	\\
painting	& 31.8	& 9.7	& -	& 15.8	& 37.7	& 25.1	\\
quickdraw	& 22.3	& 2.0	& 5.6	& -	& 13.0	& 13.2	\\
real    	& 42.4	& 12.6	& 34.5	& 19.2	& -	& 29.2	\\
sketch  	& 43.1	& 9.7	& 22.1	& 19.3	& 29.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.6	& 23.7	& 37.3	& 37.6	& 35.9	\\
infograph	& 30.2	& -	& 16.2	& 29.0	& 27.1	& 21.7	\\
painting	& 41.5	& 10.6	& -	& 33.5	& 42.5	& 32.6	\\
quickdraw	& 34.5	& 4.2	& 12.4	& -	& 23.9	& 21.6	\\
real    	& 50.1	& 13.4	& 36.9	& 35.6	& -	& 35.5	\\
sketch  	& 49.9	& 10.5	& 26.4	& 36.1	& 36.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.3	& 27.6	& 45.4	& 43.2	& 40.6	\\
infograph	& 39.0	& -	& 20.1	& 39.6	& 34.1	& 28.3	\\
painting	& 48.0	& 12.2	& -	& 42.4	& 46.9	& 37.3	\\
quickdraw	& 42.4	& 6.2	& 17.6	& -	& 32.6	& 27.9	\\
real    	& 54.4	& 15.6	& 39.1	& 44.5	& -	& 40.1	\\
sketch  	& 54.5	& 12.5	& 30.1	& 44.1	& 42.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 15.1	& 36.3	& 54.4	& 51.1	& 46.7	\\
infograph	& 51.9	& -	& 30.6	& 50.2	& 45.5	& 38.4	\\
painting	& 56.6	& 15.0	& -	& 52.9	& 53.8	& 45.0	\\
quickdraw	& 52.2	& 10.3	& 29.2	& -	& 44.5	& 38.6	\\
real    	& 61.5	& 17.8	& 44.0	& 54.1	& -	& 47.1	\\
sketch  	& 60.5	& 15.7	& 38.2	& 53.9	& 51.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.0	& 24.5	& 29.4	& 36.7	& 36.6	\\
infograph	& 22.4	& -	& 13.5	& 14.1	& 21.7	& 17.1	\\
painting	& 37.6	& 10.7	& -	& 20.4	& 40.8	& 29.1	\\
quickdraw	& 31.9	& 2.2	& 7.7	& -	& 16.6	& 16.2	\\
real    	& 47.5	& 13.3	& 37.0	& 24.4	& -	& 32.9	\\
sketch  	& 49.8	& 10.7	& 27.3	& 25.9	& 34.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.3	& 29.9	& 46.5	& 44.8	& 41.4	\\
infograph	& 39.0	& -	& 19.2	& 37.7	& 32.2	& 26.6	\\
painting	& 48.6	& 11.7	& -	& 42.0	& 45.9	& 36.6	\\
quickdraw	& 46.5	& 5.2	& 18.0	& -	& 32.6	& 27.9	\\
real    	& 56.0	& 14.5	& 39.8	& 45.0	& -	& 39.9	\\
sketch  	& 55.9	& 12.0	& 32.2	& 45.0	& 42.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.9	& 34.9	& 53.3	& 49.9	& 45.3	\\
infograph	& 48.5	& -	& 25.1	& 47.3	& 39.7	& 33.1	\\
painting	& 54.8	& 13.5	& -	& 50.3	& 50.4	& 41.5	\\
quickdraw	& 52.4	& 7.3	& 24.9	& -	& 41.8	& 35.3	\\
real    	& 59.5	& 16.4	& 42.4	& 52.5	& -	& 44.5	\\
sketch  	& 59.5	& 13.9	& 36.2	& 51.7	& 48.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.8	& 42.0	& 58.9	& 56.5	& 50.2	\\
infograph	& 57.2	& -	& 35.4	& 56.0	& 49.9	& 42.6	\\
painting	& 60.9	& 16.0	& -	& 57.2	& 56.2	& 48.0	\\
quickdraw	& 58.9	& 11.8	& 36.8	& -	& 52.0	& 44.2	\\
real    	& 64.9	& 18.8	& 47.2	& 58.6	& -	& 50.1	\\
sketch  	& 63.6	& 17.0	& 42.9	& 58.3	& 55.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 6.0	& 12.3	& 15.0	& 23.4	& 21.0	\\
infograph	& 10.2	& -	& 7.2	& 7.0	& 11.2	& 7.1	\\
painting	& 22.8	& 6.3	& -	& 8.3	& 28.7	& 17.1	\\
quickdraw	& 9.5	& 1.1	& 2.1	& -	& 5.1	& 4.9	\\
real    	& 35.4	& 9.2	& 26.4	& 9.8	& -	& 19.5	\\
sketch  	& 31.9	& 6.5	& 15.2	& 13.5	& 21.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 6.5	& 14.7	& 28.7	& 28.4	& 25.6	\\
infograph	& 17.4	& -	& 8.5	& 19.9	& 16.1	& 11.9	\\
painting	& 28.5	& 7.2	& -	& 23.1	& 31.8	& 22.3	\\
quickdraw	& 20.1	& 2.2	& 5.1	& -	& 12.5	& 12.1	\\
real    	& 39.7	& 9.9	& 27.1	& 24.1	& -	& 24.8	\\
sketch  	& 37.4	& 7.0	& 17.5	& 27.2	& 26.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 8.2	& 18.6	& 36.5	& 33.5	& 31.3	\\
infograph	& 24.2	& -	& 11.7	& 29.4	& 22.6	& 17.4	\\
painting	& 34.2	& 8.0	& -	& 32.7	& ??	& 27.9	\\
quickdraw	& 27.8	& 3.4	& 8.9	& -	& 20.5	& 18.6	\\
real    	& 43.4	& 11.1	& 29.6	& 33.7	& -	& 30.4	\\
sketch  	& 42.9	& 8.5	& 20.6	& 35.7	& 32.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.4	& 27.0	& 46.8	& 42.6	& 39.4	\\
infograph	& 37.1	& -	& 19.7	& 41.8	& 33.8	& 29.4	\\
painting	& 44.9	& 10.5	& -	& 44.2	& 43.3	& 36.8	\\
quickdraw	& 41.1	& 6.3	& 18.1	& -	& 32.4	& 29.7	\\
real    	& 49.8	& 13.4	& 34.0	& 45.2	& -	& 38.7	\\
sketch  	& 49.7	& 11.6	& 29.2	& 46.0	& 41.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.5	& 23.5	& 22.5	& 35.8	& 36.6	\\
infograph	& 23.9	& -	& 16.2	& 6.7	& 22.9	& 19.1	\\
painting	& 37.5	& 10.8	& -	& 8.8	& 41.8	& 29.8	\\
quickdraw	& 23.3	& 1.5	& 2.6	& -	& 9.5	& 10.9	\\
real    	& 45.2	& 12.3	& 36.3	& 12.6	& -	& 32.0	\\
sketch  	& 51.4	& 11.5	& 28.5	& 23.3	& 36.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 26.8	& 33.5	& 40.0	& 39.8	\\
infograph	& 33.3	& -	& 20.0	& 19.6	& 30.3	& 24.8	\\
painting	& 44.5	& 11.7	& -	& 21.6	& 45.8	& 34.0	\\
quickdraw	& 31.9	& 3.1	& 5.6	& -	& 16.5	& 18.9	\\
real    	& 50.8	& 13.4	& 39.1	& 30.7	& -	& 37.2	\\
sketch  	& 54.6	& 12.2	& 31.1	& 33.5	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.9	& 29.6	& 42.6	& 43.8	& 43.0	\\
infograph	& 40.6	& -	& 25.4	& 33.3	& 36.1	& 30.6	\\
painting	& 49.2	& 13.3	& -	& 32.4	& 48.9	& 38.6	\\
quickdraw	& 38.8	& 5.1	& 13.3	& -	& 22.3	& 24.8	\\
real    	& 55.3	& 15.2	& 40.7	& 39.4	& -	& 40.8	\\
sketch  	& 57.9	& 14.0	& 34.6	& 40.8	& 45.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.1	& 37.1	& 52.3	& 50.3	& 48.2	\\
infograph	& 51.4	& -	& 33.9	& 48.0	& 45.8	& 39.4	\\
painting	& 56.7	& 16.0	& -	& 46.7	& 54.6	& 44.8	\\
quickdraw	& 48.7	& 9.4	& 21.6	& -	& 38.0	& 37.4	\\
real    	& 60.2	& 17.9	& 45.4	& 51.0	& -	& 47.1	\\
sketch  	& 61.8	& 17.3	& 41.6	& 51.6	& 51.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.7	& 35.0	& 34.5	& 47.3	& 47.0	\\
infograph	& 37.9	& -	& 26.9	& 22.8	& 37.8	& 29.9	\\
painting	& 48.9	& 15.5	& -	& 28.5	& 51.0	& 43.3	\\
quickdraw	& 37.0	& 2.9	& 13.8	& -	& 27.8	& 24.1	\\
real    	& 59.6	& 17.9	& 47.9	& 36.5	& -	& 45.3	\\
sketch  	& 61.5	& 16.4	& 42.2	& 39.0	& 50.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 15.6	& 38.6	& 50.9	& 53.0	& 50.1	\\
infograph	& 48.1	& -	& 32.9	& 43.1	& 46.2	& 39.3	\\
painting	& 55.0	& 16.6	& -	& 44.8	& 56.0	& 48.3	\\
quickdraw	& 51.3	& 6.8	& 26.5	& -	& 43.0	& 36.4	\\
real    	& 65.0	& 19.4	& 49.8	& 51.7	& -	& 50.4	\\
sketch  	& 64.2	& 17.4	& 44.5	& 49.9	& 54.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 17.6	& 41.9	& 55.6	& 57.5	& 53.8	\\
infograph	& 53.2	& -	& 37.2	& 50.3	& 52.5	& 45.2	\\
painting	& 59.4	& 17.8	& -	& 52.6	& 59.9	& 51.2	\\
quickdraw	& 56.7	& 10.0	& 34.6	& -	& 51.0	& 44.5	\\
real    	& 67.6	& 20.9	& 51.8	& 56.9	& -	& 54.3	\\
sketch  	& 66.4	& 19.4	& 47.2	& 55.8	& 58.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 20.8	& 49.2	& 62.0	& 64.2	& 58.1	\\
infograph	& 61.5	& -	& 44.9	& 58.4	& 60.9	& 51.5	\\
painting	& 65.3	& 21.0	& -	& 59.5	& 66.2	& 56.9	\\
quickdraw	& 64.1	& 14.8	& 44.5	& -	& 61.1	& 52.6	\\
real    	& 71.1	& 24.2	& 56.1	& 62.9	& -	& 58.6	\\
sketch  	& 70.6	& 22.7	& 52.4	& 61.9	& 64.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.7	& 25.2	& 22.5	& 36.4	& 38.2	\\
infograph	& 24.9	& -	& 17.1	& 14.3	& 24.3	& 20.9	\\
painting	& 39.7	& 12.2	& -	& 17.7	& 44.2	& 34.1	\\
quickdraw	& 24.7	& 2.4	& 7.4	& -	& 15.2	& 15.8	\\
real    	& 47.9	& 14.7	& 40.4	& 20.2	& -	& 35.1	\\
sketch  	& 51.4	& 12.1	& 31.4	& 20.5	& 37.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.8	& 29.8	& 39.8	& 42.9	& 43.2	\\
infograph	& 38.9	& -	& 22.2	& 33.7	& 34.5	& 29.9	\\
painting	& 49.4	& 13.7	& -	& 36.0	& 50.2	& 40.4	\\
quickdraw	& 38.6	& 5.2	& 15.8	& -	& 27.4	& 25.9	\\
real    	& 56.0	& 15.8	& 43.0	& 37.9	& -	& 41.6	\\
sketch  	& 57.6	& 13.8	& 34.7	& 38.5	& 43.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.5	& 33.9	& 47.5	& 48.6	& 47.5	\\
infograph	& 47.3	& -	& 27.1	& 43.6	& 41.8	& 36.7	\\
painting	& 55.0	& 15.5	& -	& 45.1	& 54.2	& 45.2	\\
quickdraw	& 46.1	& 7.8	& 21.9	& -	& 37.1	& 33.9	\\
real    	& 59.9	& 18.0	& 45.7	& 46.3	& -	& 46.9	\\
sketch  	& 61.0	& 15.7	& 38.3	& 47.3	& 49.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 18.1	& 43.0	& 56.5	& 57.0	& 53.8	\\
infograph	& 59.5	& -	& 38.3	& 54.0	& 53.8	& 47.7	\\
painting	& 63.5	& 18.9	& -	& 55.3	& 60.9	& 52.5	\\
quickdraw	& 57.3	& 12.9	& 35.2	& -	& 49.6	& 44.8	\\
real    	& 66.3	& 21.3	& 51.2	& 56.0	& -	& 53.9	\\
sketch  	& 67.0	& 20.4	& 46.2	& 56.0	& 57.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.5	& 28.6	& 30.2	& 41.3	& 41.6	\\
infograph	& 27.8	& -	& 17.4	& 17.8	& 25.9	& 22.0	\\
painting	& 43.6	& 12.2	& -	& 23.3	& 45.9	& 35.1	\\
quickdraw	& 35.3	& 2.5	& 10.5	& -	& 19.7	& 18.3	\\
real    	& 51.2	& 14.4	& 40.9	& 25.9	& -	& 37.2	\\
sketch  	& 54.9	& 12.7	& 33.1	& 28.2	& 39.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 16.0	& 40.3	& 55.3	& 54.6	& 51.8	\\
infograph	& 55.1	& -	& 30.7	& 50.5	& 46.6	& 41.5	\\
painting	& 60.3	& 15.4	& -	& 52.6	& 56.4	& 48.6	\\
quickdraw	& 56.5	& 8.9	& 31.1	& -	& 46.1	& 41.4	\\
real    	& 64.2	& 18.0	& 47.0	& 53.3	& -	& 49.6	\\
sketch  	& 64.8	& 16.0	& 42.7	& 54.3	& 54.4	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 5.5	& 11.2	& 16.0	& 22.0	& 18.8	\\
infograph	& 9.1	& -	& 6.1	& 7.2	& 9.7	& 4.6	\\
painting	& 20.8	& 5.5	& -	& 9.6	& 27.4	& 13.8	\\
quickdraw	& 8.4	& 1.0	& 1.5	& -	& 3.8	& 4.3	\\
real    	& 35.8	& 9.4	& 27.2	& 12.6	& -	& 19.8	\\
sketch  	& 32.5	& 6.2	& 15.2	& 17.6	& 22.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 5.8	& 12.4	& 29.2	& 24.6	& 23.0	\\
infograph	& 13.9	& -	& 7.1	& 22.5	& 13.5	& 7.1	\\
painting	& 23.7	& 5.8	& -	& 25.7	& 29.0	& 15.3	\\
quickdraw	& 16.9	& 1.9	& 3.0	& -	& 9.9	& 9.6	\\
real    	& 38.6	& 9.7	& 26.5	& 26.4	& -	& 22.3	\\
sketch  	& 36.3	& 6.1	& 15.6	& 29.0	& 25.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.0	& 14.3	& 37.8	& 30.5	& 28.2	\\
infograph	& 20.8	& -	& 9.2	& 32.0	& 19.2	& 15.5	\\
painting	& 29.3	& 6.8	& -	& 33.2	& 33.3	& 24.1	\\
quickdraw	& 26.0	& 2.9	& 5.8	& -	& 16.8	& 17.6	\\
real    	& 42.9	& 10.8	& 28.9	& 34.5	& -	& 27.8	\\
sketch  	& 42.5	& 7.0	& 17.5	& 38.4	& 31.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.3	& 22.6	& 46.7	& 41.2	& 39.5	\\
infograph	& 34.2	& -	& 16.9	& 43.5	& 30.8	& 29.9	\\
painting	& 42.6	& 8.9	& -	& 45.7	& 42.7	& 37.9	\\
quickdraw	& 40.4	& 5.3	& 15.4	& -	& 30.5	& 30.6	\\
real    	& 50.1	& 12.9	& 34.3	& 46.2	& -	& 38.4	\\
sketch  	& 50.6	& 11.2	& 28.0	& 47.0	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'num_labels': '1', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.1	& 28.8	& 24.9	& 39.8	& 42.6	\\
infograph	& 27.5	& -	& 19.9	& 8.1	& 25.5	& 22.1	\\
painting	& 40.9	& 11.0	& -	& 9.7	& 43.9	& 33.5	\\
quickdraw	& 25.8	& 2.0	& 6.1	& -	& 12.7	& 15.9	\\
real    	& 48.1	& 13.1	& 41.1	& 14.4	& -	& 34.0	\\
sketch  	& 56.5	& 13.7	& 37.1	& 27.0	& 43.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'num_labels': '5', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 13.3	& 31.9	& 36.4	& 44.3	& 45.8	\\
infograph	& 39.7	& -	& 25.4	& 26.5	& 36.0	& 29.9	\\
painting	& 48.7	& 12.9	& -	& 24.5	& 49.9	& 38.0	\\
quickdraw	& 35.1	& 4.3	& 15.0	& -	& 25.8	& 24.2	\\
real    	& 54.8	& 14.4	& 43.5	& 32.7	& -	& 40.6	\\
sketch  	& 59.2	& 14.4	& 39.4	& 37.5	& 46.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'num_labels': '10', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'num_labels': '25', 'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 18.8	& 43.0	& 53.0	& 55.3	& 53.7	\\
infograph	& 58.0	& -	& 39.4	& 51.6	& 50.8	& 46.4	\\
painting	& 61.5	& 17.9	& -	& 49.9	& 57.3	& 49.6	\\
quickdraw	& 54.5	& 11.8	& 33.7	& -	& 47.2	& 42.6	\\
real    	& 64.0	& 20.0	& 49.6	& 54.0	& -	& 51.6	\\
sketch  	& 65.9	& 20.3	& 48.4	& 53.8	& 55.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

% data/NextMatch Results - SSDA.csv
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive	& DigitFive	& DigitFive	& DigitFive	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet224	& DomainNet224	& DomainNet224	& DomainNet224	\\
& 25	& 10	& 1	& 5	& 10	& 5	& 25	& 1	& 25	& 5	& 1	& 10	\\
\\
\midrule
BaselineBN	& 89.4	& 85.7	& 73.4	& 81.0	& 34.0	& 28.6	& 42.1	& 20.8	& 47.6	& 33.8	& 25.3	& 39.3	\\
MCD     	& nan	& nan	& nan	& nan	& 24.3	& 19.5	& 33.2	& 13.8	& 32.5	& 17.8	& 13.5	& 23.1	\\
NoisyStudent	& 80.5	& 76.4	& 72.8	& 75.3	& 33.6	& 28.6	& 41.4	& 22.8	& 46.0	& 33.0	& 26.0	& nan	\\
FixMatch+	& 97.9	& 98.1	& 83.1	& 97.8	& 39.6	& 34.2	& 46.1	& 24.8	& nan	& nan	& 28.3	& 44.1	\\
AdaMatch	& 97.7	& 98.0	& 97.9	& 98.0	& 40.6	& 36.5	& 46.4	& 30.4	& 52.8	& 42.3	& 34.8	& 46.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}



%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 10.1	\\
svhn    	& 39.8	\\
syndigit	& 99.2	\\
usps    	& 96.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 98.0	\\
mnistm  	& 97.3	\\
svhn    	& 96.3	\\
syndigit	& 99.1	\\
usps    	& 95.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 97.1	\\
svhn    	& 95.7	\\
syndigit	& 99.4	\\
usps    	& 96.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.2	\\
syndigit	& 97.8	\\
usps    	& 97.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 64.4	\\
mnistm  	& 14.6	\\
svhn    	& 16.9	\\
syndigit	& 41.0	\\
usps    	& 63.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 83.2	\\
mnistm  	& 29.9	\\
svhn    	& 36.5	\\
syndigit	& 77.9	\\
usps    	& 81.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 91.1	\\
mnistm  	& 51.5	\\
svhn    	& 54.0	\\
syndigit	& 83.5	\\
usps    	& 88.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 95.3	\\
mnistm  	& 78.3	\\
svhn    	& 69.5	\\
syndigit	& 94.4	\\
usps    	& 94.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.8	\\
mnistm  	& 9.9	\\
svhn    	& 31.5	\\
syndigit	& 37.9	\\
usps    	& 80.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 97.4	\\
svhn    	& 82.2	\\
syndigit	& 99.1	\\
usps    	& 97.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.3	\\
mnistm  	& 98.9	\\
svhn    	& 96.8	\\
syndigit	& 99.5	\\
usps    	& 97.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	\\
mnistm  	& 98.8	\\
svhn    	& 95.9	\\
syndigit	& 99.4	\\
usps    	& 97.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 61.6	\\
mnistm  	& 10.4	\\
svhn    	& 8.5	\\
syndigit	& 9.7	\\
usps    	& 46.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 90.9	\\
mnistm  	& 18.8	\\
svhn    	& 11.5	\\
syndigit	& 40.5	\\
usps    	& 92.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 94.8	\\
mnistm  	& 80.4	\\
svhn    	& 31.4	\\
syndigit	& 92.4	\\
usps    	& 92.8	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.1	\\
mnistm  	& 94.4	\\
svhn    	& 82.3	\\
syndigit	& 96.6	\\
usps    	& 94.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=1}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 71.2	\\
mnistm  	& 13.1	\\
svhn    	& 16.2	\\
syndigit	& 40.8	\\
usps    	& 75.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=5}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 91.0	\\
mnistm  	& 29.6	\\
svhn    	& 41.9	\\
syndigit	& 84.5	\\
usps    	& 89.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=10}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 96.8	\\
mnistm  	& 59.9	\\
svhn    	& 62.0	\\
syndigit	& 90.9	\\
usps    	& 92.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=25}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 97.9	\\
mnistm  	& 90.5	\\
svhn    	& 80.0	\\
syndigit	& 95.9	\\
usps    	& 96.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_25 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.5	\\
infograph	& 1.5	\\
painting	& 3.9	\\
quickdraw	& 18.7	\\
real    	& 8.3	\\
sketch  	& 6.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 41.5	\\
infograph	& 4.0	\\
painting	& 13.0	\\
quickdraw	& 42.0	\\
real    	& 28.6	\\
sketch  	& 25.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 51.8	\\
infograph	& 5.8	\\
painting	& 21.7	\\
quickdraw	& 51.5	\\
real    	& 42.4	\\
sketch  	& 36.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 62.6	\\
infograph	& 10.3	\\
painting	& 39.5	\\
quickdraw	& 59.8	\\
real    	& 56.5	\\
sketch  	& 49.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 7.4	\\
infograph	& 1.3	\\
painting	& 3.4	\\
quickdraw	& 14.5	\\
real    	& 7.0	\\
sketch  	& 5.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 26.6	\\
infograph	& 3.3	\\
painting	& 9.1	\\
quickdraw	& 33.1	\\
real    	& 20.1	\\
sketch  	& 16.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 37.9	\\
infograph	& 5.0	\\
painting	& 13.5	\\
quickdraw	& 42.6	\\
real    	& 31.1	\\
sketch  	& 26.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 53.2	\\
infograph	& 8.2	\\
painting	& 28.0	\\
quickdraw	& 53.8	\\
real    	& 46.2	\\
sketch  	& 41.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=5}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=10}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=25}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 2.3	\\
infograph	& 0.9	\\
painting	& 1.7	\\
quickdraw	& 7.5	\\
real    	& 3.0	\\
sketch  	& 1.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 9.2	\\
infograph	& 1.9	\\
painting	& 3.8	\\
quickdraw	& 25.1	\\
real    	& 9.3	\\
sketch  	& 4.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 16.4	\\
infograph	& 3.4	\\
painting	& 7.1	\\
quickdraw	& 35.7	\\
real    	& 16.2	\\
sketch  	& 10.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 31.8	\\
infograph	& 5.7	\\
painting	& 15.1	\\
quickdraw	& 47.4	\\
real    	& 28.8	\\
sketch  	& 27.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=1}} \\
\midrule
\\
\midrule
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 36.4	\\
infograph	& 3.9	\\
painting	& 13.6	\\
quickdraw	& 39.8	\\
real    	& 27.8	\\
sketch  	& 24.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.3	\\
infograph	& 5.6	\\
painting	& 20.9	\\
quickdraw	& 49.6	\\
real    	& 41.5	\\
sketch  	& 35.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 60.8	\\
infograph	& 9.7	\\
painting	& 38.8	\\
quickdraw	& 59.4	\\
real    	& 55.2	\\
sketch  	& 48.5	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_25 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.2	\\
infograph	& 1.5	\\
painting	& 4.0	\\
quickdraw	& 18.9	\\
real    	& 8.5	\\
sketch  	& 5.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_1 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 36.5	\\
infograph	& 3.6	\\
painting	& 13.3	\\
quickdraw	& 41.7	\\
real    	& 26.9	\\
sketch  	& 21.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_5 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 46.4	\\
infograph	& 5.8	\\
painting	& 20.8	\\
quickdraw	& 49.9	\\
real    	& 37.9	\\
sketch  	& 29.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_10 }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 56.2	\\
infograph	& 9.3	\\
painting	& 33.3	\\
quickdraw	& 57.7	\\
real    	& 50.3	\\
sketch  	& 41.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_25 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 6.9	\\
infograph	& 1.4	\\
painting	& 3.1	\\
quickdraw	& 13.2	\\
real    	& 6.6	\\
sketch  	& 4.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_1 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 23.6	\\
infograph	& 3.2	\\
painting	& 9.1	\\
quickdraw	& 31.2	\\
real    	& 18.2	\\
sketch  	& 13.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_5 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 33.9	\\
infograph	& 4.8	\\
painting	& 14.2	\\
quickdraw	& 40.3	\\
real    	& 28.2	\\
sketch  	& 22.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_10 }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.2	\\
infograph	& 7.8	\\
painting	& 25.7	\\
quickdraw	& 51.1	\\
real    	& 41.5	\\
sketch  	& 34.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_25 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 9.7	\\
infograph	& 1.4	\\
painting	& 3.9	\\
quickdraw	& 17.1	\\
real    	& 7.5	\\
sketch  	& 6.0	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_1 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 37.6	\\
infograph	& 3.5	\\
painting	& 13.1	\\
quickdraw	& 42.3	\\
real    	& 27.2	\\
sketch  	& 21.1	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_5 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 48.1	\\
infograph	& 5.3	\\
painting	& 18.9	\\
quickdraw	& 50.9	\\
real    	& 39.0	\\
sketch  	& 30.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_10 }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 57.2	\\
infograph	& 8.8	\\
painting	& 32.7	\\
quickdraw	& 58.0	\\
real    	& 50.5	\\
sketch  	& 41.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_25 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 3.0	\\
infograph	& 1.0	\\
painting	& 1.8	\\
quickdraw	& 7.8	\\
real    	& 3.5	\\
sketch  	& 1.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_1 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 10.5	\\
infograph	& 2.3	\\
painting	& 5.0	\\
quickdraw	& 25.1	\\
real    	& 11.3	\\
sketch  	& 6.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_5 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 19.6	\\
infograph	& 3.5	\\
painting	& 9.5	\\
quickdraw	& 35.1	\\
real    	& 18.7	\\
sketch  	& 13.6	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_10 }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 34.7	\\
infograph	& 5.6	\\
painting	& 17.3	\\
quickdraw	& 47.1	\\
real    	& 32.3	\\
sketch  	& 27.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_25 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '1'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=1}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 8.7	\\
infograph	& 1.5	\\
painting	& 4.1	\\
quickdraw	& 16.7	\\
real    	& 7.6	\\
sketch  	& 5.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_1 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '5'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=5}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 31.8	\\
infograph	& 3.5	\\
painting	& 11.8	\\
quickdraw	& 37.1	\\
real    	& 24.3	\\
sketch  	& 17.9	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_5 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '10'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=10}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 42.3	\\
infograph	& 5.3	\\
painting	& 18.6	\\
quickdraw	& 46.7	\\
real    	& 35.6	\\
sketch  	& 27.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_10 }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64', 'num_labels': '25'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=25}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& 54.6	\\
infograph	& 8.7	\\
painting	& 31.7	\\
quickdraw	& 57.4	\\
real    	& 49.4	\\
sketch  	& 40.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_25 }
\end{table}

% ['data/NextMatch Results - SSL.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrrrrrrrr}
\toprule
& DigitFive	& DigitFive	& DigitFive	& DigitFive	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet64	& DomainNet224	& DomainNet224	& DomainNet224	& DomainNet224	\\
& 10	& 5	& 25	& 1	& 25	& 5	& 1	& 10	& 10	& 5	& 25	& 1	\\
\\
\midrule
BaselineBN	& 73.7	& 61.9	& 86.4	& 40.0	& 34.9	& 16.5	& 5.9	& 23.9	& 26.2	& 18.1	& 38.5	& 6.5	\\
MCD     	& 78.4	& 50.8	& 93.0	& 27.4	& 27.5	& 10.2	& 3.1	& 16.7	& 14.9	& 8.9	& 26.0	& 2.8	\\
NoisyStudent	& 80.5	& 67.4	& 92.1	& 43.3	& 40.3	& 21.1	& 7.3	& 29.3	& 33.6	& 24.2	& 45.4	& nan	\\
FixMatch+	& 98.3	& 94.8	& 98.1	& 51.5	& 41.5	& 24.1	& 7.6	& 32.1	& nan	& nan	& nan	& nan	\\
AdaMatch	& 97.6	& 97.2	& 97.6	& 68.6	& 41.4	& 23.8	& 8.1	& 31.7	& 34.9	& 25.7	& 46.4	& 8.2	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 AdaMatch nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 14.8	& 35.3	& 26.8	& 46.5	& 46.5	\\
infograph	& 21.7	& -	& 11.7	& 0.3	& 20.0	& 0.2	\\
painting	& 45.3	& 13.5	& -	& 13.2	& 48.1	& 41.0	\\
quickdraw	& 33.6	& 2.4	& 10.1	& -	& 19.1	& 21.1	\\
real    	& 56.0	& 16.6	& 47.6	& 22.9	& -	& 42.4	\\
sketch  	& 60.2	& 17.0	& 42.9	& 34.2	& 49.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Baseline nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.4	& 23.4	& 12.1	& 33.4	& 34.9	\\
infograph	& 16.2	& -	& 13.8	& 0.9	& 16.5	& 11.5	\\
painting	& 33.6	& 11.2	& -	& 1.0	& 41.2	& 25.7	\\
quickdraw	& 11.2	& 0.8	& 2.5	& -	& 5.5	& 7.1	\\
real    	& 43.4	& 13.7	& 39.4	& 2.1	& -	& 29.6	\\
sketch  	& 47.9	& 11.0	& 28.7	& 3.8	& 33.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FixMatchDA nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.6	& 26.4	& 11.2	& 37.6	& 37.8	\\
infograph	& 15.8	& -	& 6.5	& 0.6	& 8.6	& 11.4	\\
painting	& 39.0	& 11.6	& -	& 4.2	& 42.7	& 31.4	\\
quickdraw	& 15.8	& 1.3	& 5.0	& -	& 11.5	& 12.2	\\
real    	& 48.1	& 13.8	& 39.8	& 7.3	& -	& 33.4	\\
sketch  	& 50.3	& 11.8	& 30.7	& 11.8	& 34.2	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 MCD nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.7	& 15.2	& 15.2	& 25.8	& 23.4	\\
infograph	& 9.2	& -	& 7.0	& 1.6	& 11.2	& 6.5	\\
painting	& 25.6	& 7.0	& -	& 5.3	& 32.1	& 18.8	\\
quickdraw	& 7.4	& 0.7	& 0.7	& -	& 1.6	& 4.1	\\
real    	& 38.4	& 10.5	& 32.4	& 7.7	& -	& 22.9	\\
sketch  	& 37.2	& 8.2	& 22.9	& 14.7	& 26.7	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 NoisyStudent nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.9	& 28.5	& 20.4	& 39.5	& 42.3	\\
infograph	& 24.5	& -	& 18.9	& 3.1	& 23.9	& 18.3	\\
painting	& 37.6	& 11.4	& -	& 3.4	& 40.9	& 30.9	\\
quickdraw	& 20.9	& 1.0	& 2.7	& -	& 8.7	& 13.2	\\
real    	& 47.8	& 13.7	& 39.8	& 7.7	& -	& 32.6	\\
sketch  	& 55.2	& 14.8	& 37.1	& 22.8	& 41.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_NoisyStudent_None }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 AdaMatch nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 12.2	& 29.3	& 27.9	& 40.8	& 40.6	\\
infograph	& 22.1	& -	& 18.5	& 6.2	& 24.2	& 19.8	\\
painting	& 39.6	& 11.7	& -	& 12.6	& 43.4	& 34.9	\\
quickdraw	& 24.6	& 2.4	& 8.4	& -	& 16.4	& 15.5	\\
real    	& 52.2	& 15.0	& 41.6	& 13.3	& -	& 38.6	\\
sketch  	& 53.4	& 13.6	& 35.6	& 25.4	& 41.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Baseline nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.5	& 19.0	& 6.3	& 29.4	& 29.9	\\
infograph	& 12.9	& -	& 10.8	& 0.6	& 14.0	& 9.5	\\
painting	& 27.3	& 9.3	& -	& 1.0	& 36.3	& 21.8	\\
quickdraw	& 10.3	& 0.8	& 1.9	& -	& 4.8	& 5.9	\\
real    	& 39.3	& 11.9	& 34.6	& 2.2	& -	& 25.5	\\
sketch  	& 40.9	& 8.5	& 20.4	& 3.3	& 26.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FixMatchDA nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.2	& 24.6	& 14.6	& 35.7	& 35.3	\\
infograph	& 17.9	& -	& 14.3	& 2.2	& 18.7	& 14.2	\\
painting	& 34.7	& 10.7	& -	& 4.2	& 39.7	& 27.7	\\
quickdraw	& 23.7	& 1.4	& 5.1	& -	& 11.2	& 10.2	\\
real    	& 45.4	& 13.5	& 37.4	& 6.6	& -	& 30.7	\\
sketch  	& 48.1	& 10.3	& 26.6	& 10.4	& 31.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 MCD nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 7.5	& 15.9	& 12.9	& 26.2	& 25.6	\\
infograph	& 11.3	& -	& 9.4	& 2.3	& 13.3	& 8.6	\\
painting	& 25.8	& 7.5	& -	& 4.3	& 32.1	& 21.4	\\
quickdraw	& 8.0	& 0.6	& 0.6	& -	& 1.6	& 4.6	\\
real    	& 37.2	& 10.1	& 29.8	& 6.8	& -	& 22.9	\\
sketch  	& 37.3	& 7.8	& 20.2	& 11.6	& 25.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 NoisyStudent nlab=None}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 10.9	& 24.3	& 18.9	& 35.4	& 36.8	\\
infograph	& 21.2	& -	& 16.9	& 2.6	& 21.8	& 16.0	\\
painting	& 36.1	& 11.7	& -	& 3.6	& 41.5	& 28.5	\\
quickdraw	& 19.0	& 0.9	& 1.5	& -	& 6.8	& 7.2	\\
real    	& 44.0	& 13.8	& 38.3	& 6.6	& -	& 30.6	\\
sketch  	& 50.0	& 12.0	& 30.4	& 18.2	& 36.0	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_NoisyStudent_None }
\end{table}

%% run {'algorithm': 'AdaMatch', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 AdaMatch nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 96.6	& 97.6	\\
mnistm  	& 96.7	\\
svhn    	& 99.3	\\
syndigit	& 96.9	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_AdaMatch_None }
\end{table}

%% run {'algorithm': 'Baseline', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Baseline nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 54.3	& 55.0	& 76.0	& 96.3	\\
mnistm  	& 96.5	& -	& 52.4	& 81.8	& 88.1	\\
svhn    	& 40.4	& 32.0	& -	& 86.3	& 39.9	\\
syndigit	& 67.7	& 30.0	& 79.7	& -	& 70.5	\\
usps    	& 78.6	& 27.3	& 31.9	& 64.8	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Baseline_None }
\end{table}

%% run {'algorithm': 'FixMatchDA', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FixMatchDA nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 99.2	& 97.0	& 97.9	\\
mnistm  	& 96.8	\\
svhn    	& 99.2	\\
syndigit	& 96.9	\\
usps    	& 99.3	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FixMatchDA_None }
\end{table}

%% run {'algorithm': 'MCD', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 MCD nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& 13.1	& 9.7	& 91.2	\\
mnistm  	& 16.9	\\
svhn    	& 81.3	\\
syndigit	& 84.3	\\
usps    	& 94.4	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_MCD_None }
\end{table}

%% run {'algorithm': 'NoisyStudent', 'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 NoisyStudent nlab=None}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 30.4	& 51.4	& 81.8	& 97.2	\\
mnistm  	& 99.2	& -	& 63.0	& 89.0	& 97.0	\\
svhn    	& 82.8	& 45.2	& -	& 98.9	& 83.9	\\
syndigit	& 92.6	& 50.5	& 90.0	& -	& 87.1	\\
usps    	& 95.5	& 25.2	& 30.0	& 75.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_NoisyStudent_None }
\end{table}

% ['data/NextMatch Results - DA - DigitFive (MCD).csv', 'data/NextMatch Results - DA.csv']
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrr}
\toprule
& DigitFive	& DomainNet64	& DomainNet224	\\
& 1	& 1	& 1	\\
\\
\midrule
BaselineBN	& 62.5	& 15.8	& 18.9	\\
MCD     	& 55.9	& 14.9	& 14.9	\\
NoisyStudent	& 73.3	& 21.4	& 23.9	\\
FixMatch+	& 98.1	& 20.6	& 20.8	\\
AdaMatch	& 97.9	& 26.0	& 28.7	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{}
\end{table}

%% run {'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 FSL}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 9.3	& 19.3	& 15.0	& 30.1	& 31.9	\\
infograph	& 14.7	& -	& 11.2	& 2.1	& 15.3	& 11.4	\\
painting	& 29.8	& 9.1	& -	& 2.8	& 37.6	& 24.0	\\
quickdraw	& 14.5	& 0.8	& 0.9	& -	& 4.9	& 5.9	\\
real    	& 42.5	& 13.2	& 36.9	& 6.5	& -	& 27.9	\\
sketch  	& 43.0	& 9.2	& 22.4	& 13.6	& 28.3	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_FSL }
\end{table}

%% run {'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 FSL}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 11.6	& 24.6	& 16.4	& 35.6	& 38.1	\\
infograph	& 21.3	& -	& 16.3	& 3.4	& 21.8	& 17.1	\\
painting	& 37.6	& 11.5	& -	& 5.4	& 44.4	& 31.4	\\
quickdraw	& 15.3	& 0.8	& 1.7	& -	& 5.4	& 8.7	\\
real    	& 48.0	& 15.8	& 44.1	& 8.0	& -	& 34.5	\\
sketch  	& 50.0	& 11.7	& 31.7	& 17.1	& 36.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_FSL }
\end{table}

%% run {'dataset': 'domainnet64'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet64 Oracle}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 31.6	& 60.0	& 70.7	& 70.7	& 62.5	\\
infograph	& 70.0	& -	& 58.2	& 69.8	& 69.2	& 60.1	\\
painting	& 71.9	& 32.3	& -	& 70.3	& 71.0	& 62.3	\\
quickdraw	& 70.2	& 29.5	& 58.3	& -	& 69.1	& 60.3	\\
real    	& 73.5	& 33.8	& 61.9	& nan	& -	& 63.3	\\
sketch  	& 72.3	& 31.9	& 60.2	& 70.6	& 70.1	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet64_Oracle }
\end{table}

%% run {'dataset': 'domainnet224'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{domainnet224 Oracle}} \\
\midrule
& clipart	& infograph	& painting	& quickdraw	& real	& sketch	\\
\midrule
clipart 	& -	& 38.8	& 65.9	& 71.9	& 74.8	& 69.0	\\
infograph	& 75.8	& -	& 65.7	& 71.4	& 74.5	& 67.7	\\
painting	& 76.9	& 39.1	& -	& 71.8	& 75.6	& 68.4	\\
quickdraw	& 74.5	& 35.7	& 63.4	& -	& 72.7	& 66.2	\\
real    	& 77.8	& 40.6	& 67.7	& 71.9	& -	& 69.2	\\
sketch  	& 77.3	& 39.5	& 66.1	& 72.1	& 74.5	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_domainnet224_Oracle }
\end{table}

%% run {'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 FSL}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 23.3	& 33.9	& 72.9	& 95.9	\\
mnistm  	& 98.7	& -	& 43.9	& 83.0	& 96.2	\\
svhn    	& 72.1	& 37.3	& -	& 98.2	& 75.2	\\
syndigit	& 88.5	& 30.6	& 80.1	& -	& 78.0	\\
usps    	& 81.8	& 15.0	& 23.3	& 69.6	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_FSL }
\end{table}

%% run {'dataset': 'digitfive32'}
\begin{table} % AUTOGENERATED TABLE, DO NOT EDIT
\centering
\begin{tabular}{l|rrrrrr}
\toprule
\multicolumn{7}{c} {\textbf{digitfive32 Oracle}} \\
\midrule
& mnist	& mnistm	& svhn	& syndigit	& usps	\\
\midrule
mnist   	& -	& 99.2	& 97.5	& 99.9	& 98.1	\\
mnistm  	& 99.5	& -	& 97.6	& 99.9	& 98.0	\\
svhn    	& 99.4	& 99.1	& -	& 99.9	& 97.6	\\
syndigit	& 99.5	& 99.1	& 97.6	& -	& 97.6	\\
usps    	& 99.5	& 99.2	& 97.5	& 99.9	& -	\\
\bottomrule
\end{tabular}
\caption{TODO}
\label{ tab:da_digitfive32_Oracle }
\end{table}

